Scalable Frame Sampling for Video Classification: A Semi-Optimal Policy Approach with Reduced Search Space

Given a video with $T$ frames, frame sampling is a task to select $N \ll T$ frames, so as to maximize the performance of a fixed video classifier. Not just brute-force search, but most existing methods suffer from its vast search space of $\binom{T}{N}$, especially when $N$ gets large. To address this challenge, we introduce a novel perspective of reducing the search space from $O(T^N)$ to $O(T)$. Instead of exploring the entire $O(T^N)$ space, our proposed semi-optimal policy selects the top $N$ frames based on the independently estimated value of each frame using per-frame confidence, significantly reducing the computational complexity. We verify that our semi-optimal policy can efficiently approximate the optimal policy, particularly under practical settings. Additionally, through extensive experiments on various datasets and model architectures, we demonstrate that learning our semi-optimal policy ensures stable and high performance regardless of the size of $N$ and $T$.

==> arXiv-2409.05260v4/figures/acc_vs_eff.tex <==
\begin{figure}
  \includegraphics[width=6.5cm]{files/performance.png}
  \includegraphics[width=6.5cm]{files/TimeSformer_acc_vs_eff.png}
  \vspace{0.2cm}
  \caption{\textbf{Mean Average Precision (\%) vs. efficiency (GFLOPs) on ActivityNet.} With a ResNet classifier (\emph{left}), OCSampler~\cite{lin2022ocsampler} is the second best after ours. With TimeSformer in (\emph{right}), however, it even underperforms than the uniform sampling. On the other hand, our approach outperforms all baselines with both ResNet50 and TimeSformer.}
  \label{fig:acc_vs_eff}
\end{figure}


\iffalse
\begin{figure}
  %\vspace{-0.6cm}
  \begin{tabular}[c]{cc}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth]{files/performance.png}
      \caption{ResNet50}
      \label{fig:resnet_acc_vs_eff}
    \end{subfigure}
    \\
    % \hspace{-1cm}
    % \vspace{1cm}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth]{files/TimeSformer_acc_vs_eff.png}
      \caption{TimeSformer}
      \label{fig:timesformer_acc_vs_eff}
    \end{subfigure}
  \end{tabular}
  % \hspace{-1cm}
  \caption{\textbf{Mean Average Precision (\%) vs. efficiency (GFLOPs) on ActivityNet.} With a ResNet classifier in (a), OCSampler~\cite{lin2022ocsampler} is the second best after ours. With TimeSformer in (b), however, it even underperforms than the uniform sampling. On the other hand, our approach outperforms all baselines with both ResNet50 and TimeSformer.}
  \label{fig:acc_vs_eff}
  % \vspace{-0.5cm}
\end{figure}

\fi


% \begin{figure}
%     \centering
%     \includegraphics[width=0.25\textwidth]{files/ResNet50_acc_vs_eff.png}
%     \includegraphics[width=0.25\textwidth]{files/TimeSformer_acc_vs_eff.png}
%     % \vspace{-60pt}
%     \caption{\textbf{Efficiency (GFLOPS) vs. mean Average Precision (\%) on ActivityNet.}  }
%     \label{fig:confidence-based sampler}
% \end{figure}\textbf{}

==> arXiv-2409.05260v4/figures/anet_uni_oc_kd_tn_comparison.tex <==
\begin{figure}[h]
    % \vspace{}
    \centering
    \includegraphics[width=\textwidth]{files/anet_r50_uni_oc_kd_tn_comparison.png}
    \caption{\textbf{Performance by sampler across N/T.}}
    \vspace{-0.4cm}
    \label{fig:anet_comparison}
\end{figure}

==> arXiv-2409.05260v4/figures/confidence_based_sampler.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{files/confidence_based_sampling.drawio.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \captionof{figure}{\textbf{Illustration of the Semi-Optimal Policy $\bm{\pi_s}$.} We briefly illustrate how $\pi_s$ works on two different architecture. The numbers in the pink and blue boxes represent the frame indices sampled with ResNet50 and TimeSformer as the backbone, respectively, when $N=6$.}
        \label{fig:confidence-based sampler}
    \end{minipage}
    %\vspace{-0.6cm}
\end{figure}

% We illustrate a significantly different distribution of label confidences over frames for a basketball cheer-leading video between ResNet50~\cite{he2016resnet} and TimeSformer~\cite{bertasius2021timesformer}.

==> arXiv-2409.05260v4/figures/large_tn_table_graph.tex <==
\begin{figure}
    \begin{minipage}[b]{0.56\linewidth}
        \centering
            \centering
            \renewcommand{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{
            \begin{tabular}{@{}l|l|l|ccc@{}}
            \toprule
            \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{$N$~/~$T$} \\
            % \cmidrule(l){4-6}
                                         &                           &         & 8~/~30          & 16~/~60         & 32~/~100         \\ 
            \midrule
            \multirow{6}{*}{ActivityNet} & \multirow{3}{*}{ResNet50}      & Uniform           & 77.1\%       & 79.4\%       & 80.4\%       \\
                                         % &                              & Random            & 75.68        & 78.97        & 80.12        \\
                                         &                              & OCSampler         & 78.0\%        & 79.1\%        & 80.1\%        \\
                                         &                              & \textbf{SOSampler}         & \textbf{78.7\%}        & \textbf{80.2\%}        & \textbf{81.1\%}        \\ 
            \cmidrule(l){2-6}
                                         & \multirow{3}{*}{TimeSformer}  & Uniform           & 88.5\%        & 89.9\%        & 90.3\%        \\
                                         % &                              & Random            & 87.48        & 89.07        & 90.06        \\
                                         &                              & OCSampler         & 85.0\%        & 85.3\%        & 84.5\%        \\
                                         &                              & \textbf{SOSampler}         & \textbf{89.5\%}        & \textbf{90.1\%}        & \textbf{90.5\%}        \\ 
            \midrule
            \multirow{6}{*}{Mini-Sports1M} & \multirow{3}{*}{ResNet50} & Uniform  & 46.9\% & 48.8\% & 49.1\% \\
                                         % &  & Random  & 46.09 & 48.69 & 48.92 \\
                                         &  & OCSampler  & 48.6\% & 49.6\% & 50.0\% \\
                                         &  & \textbf{SOSampler}  & \textbf{50.0\%} & \textbf{51.1\%} & \textbf{51.5\%} \\
            \cmidrule(l){2-6}
                                         & \multirow{3}{*}{TimeSformer} & Uniform  & 53.9\% & 55.6\% & 56.8\% \\
                                         % &  & Random  & 52.94 & 56.55 & 57.79 \\
                                         &  & OCSampler & 48.9\% & 49.6\% & 50.0\% \\
                                         &  & \textbf{SOSampler} & \textbf{55.1\%} & \textbf{56.9\%} & \textbf{57.8\%} \\
            \bottomrule
            \end{tabular}
            }
            \vspace{0.3cm}
            \captionof{table}{\textbf{Experiment on long videos for large $N$ and $T$}. The best performing model is \textbf{bold-faced}.}
            \label{tab:large_tn}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.41\linewidth}
        \centering
        % \vspace{-5cm}
        \includegraphics[width=\textwidth]{files/anet_r50_uni_oc_kd_tn_comparison.png}
        % \vspace{-0.8cm}
        \caption{\textbf{Performance by sampler across N/T on ActivityNet-v1.3.}}
        \label{fig:anet_tn_graph}
    \end{minipage}
    % \vspace{-0.6cm}
\end{figure}


==> arXiv-2409.05260v4/figures/mutual_infomation.tex <==
\begin{figure}[t]
  \centering
  % \includegraphics[width=0.49\textwidth]{files/anet_resnet_fps_coolwarm.pdf}
  % \includegraphics[width=0.49\textwidth]{files/anet_timesformer_fps_coolwarm.pdf}
  \includegraphics[width=\textwidth]{files/anet_fps.drawio.pdf}
  % \includegraphics[width=2.5cm]{files/diff_frame.png}
  \vspace{-0.2cm}
  \caption{\textbf{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$} with kernel density estimate.}
  %\captionof{figure}{\textbf{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$.} The plot on the left shows the results for ResNet features, while the plot on the right shows the results for TimeSformer features.}
  \label{fig:mutual_info}
  %\vspace{-0.2cm}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.66\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{files/anet_fps.drawio.pdf}
%         \caption{\textbf{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$} with kernel density estimate.}
%         \label{fig:mutual_info}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{files/confidence_based_sampling.drawio.pdf}
%         \caption{\textbf{Illustration of the Semi-Optimal Policy $\bm{\pi_s}$.} We briefly illustrate how $\pi_s$ works on two different architectures. The numbers in the pink and blue boxes represent the frame indices sampled with ResNet50 and TimeSformer as the backbone, respectively, when $N=6$.}
%         \label{fig:confidence-based sampler}
%     \end{subfigure}
% \end{figure}

% \begin{figure}[htb]
%     \centering
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{files/anet_resnet_fps_0.1_0.5_1_5_15_30.png}
%         \caption{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$ of ResNet50}
%         \label{fig:mu}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{files/anet_timesformer_fps_0.1_0.5_1_5_15_30.png}
%         \caption{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$ of TimeSformer}
%         \label{fig:image2}
%     \end{minipage}
% \end{figure}

% \iffalse
%   % \vspace{-0.6cm}
%   \begin{tabular}[c]{ccc}
%     \begin{subfigure}[b]{0.3\linewidth}
%       \includegraphics[width=\textwidth]{files/30_fps.png}
%       \caption{}
%       \label{fig:pxy_dist_30fps}
%     \end{subfigure}
%     & 
%     % \vspace{1cm}
%     \begin{subfigure}[b]{0.3\linewidth}
%       \includegraphics[width=\textwidth]{files/1_fps.png}
%       \caption{}
%       \label{fig:pxy_dist_1fps}
%     \end{subfigure}
%     & 
%     % \vspace{1cm}
%     \begin{subfigure}[b]{0.3\linewidth}
%       \includegraphics[width=\textwidth]{files/diff_frame.png}
%       \caption{}
%       \label{fig:pxy_dist_diff}
%     \end{subfigure}
%   \end{tabular}
%   %\hspace{-1cm}
%   % \vspace{-0.3cm}
%   \caption{\textbf{Distribution of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$.} (a) two consecutive frames at 30 fps, (b) two consecutive frames at 1 fps, (c) two frames from different videos.}
%   \label{fig:mutual_info}
%   % \vspace{-0.5cm}
% \end{figure}

% \fi

==> arXiv-2409.05260v4/figures/overview.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{files/sosampler.drawio_compressed.pdf}
    \vspace{0pt}
    \vspace{-0.4cm}
    \caption{\textbf{SOSampler Algorithm.} SOSampler consists of a sampler $S_\text{SO}$ and a classifier $f_c$, which can be any model architecture.}
    % Given the input frames, the sampler $S_\text{so}$ predicts labels $\bm{\hat{y}_s}$ with importance scores $\bm{\hat{p}_s}$ for each of them.
    %the sampler $S_\text{KD}$ selects the frames that will be fed into the classifier $f_c$ based on the importance score.
    %receives downsampled input frames and outputs the label predictions $\bm{\hat{y}_s}$ and predicted importance scores $\bm{\hat{p}_s}$.
    % For training, it minimizes cross-entropy loss between $\bm{\hat{y}_s}$ and the actual labels $\bm{y}$ and a ranking loss between $\bm{\hat{p}_s}$ and the importance score $\bm{p_s}$ from the frozen classifier $f_c$.
    % At inference, it selects the required number of frames among the input frames
    % based on the label prediction scores of each frame. 
    %At inference, the sampler simply takes the downsampled input frames and selects the required number of frames to be taken by the classifier $f_c$
    % in the order of the highest importance score.}
    \label{fig:overview}
    %\vspace{-0.3cm}
\end{figure}

==> arXiv-2409.05260v4/figures/qualitative_analysis.tex <==
\begin{figure*}[th!]
    \centering
    \includegraphics[width=.74\linewidth]{files/sampled_minus.pdf}
    \vspace{0.2cm}
    \caption{\textbf{Qualitative Examples on ActivityNet-v1.3.} 
    Our approach samples only frames that are relevant to label action and contribute to downstream tasks, and discard irrelevant frames. Label action is denoted under each clip.}
    \label{fig:qualitative_analysis}
    \vspace{-0.2cm}
\end{figure*}

==> arXiv-2409.05260v4/sec/0_abstract.tex <==
    \begin{abstract}
Given a video with $T$ frames, frame sampling is a task to select $N \ll T$ frames, so as to maximize the performance of a fixed video classifier.
Not just brute-force search, but most existing methods suffer from its vast search space of $\binom{T}{N}$, especially when $N$ gets large.
To address this challenge, we introduce a novel perspective of reducing the search space from $O(T^N)$ to $O(T)$.
Instead of exploring the entire $O(T^N)$ space, our proposed semi-optimal policy selects the top $N$ frames based on the independently estimated value of each frame using per-frame confidence, significantly reducing the computational complexity.
We verify that our semi-optimal policy can efficiently approximate the optimal policy, particularly under practical settings. Additionally, through extensive experiments on various datasets and model architectures, we demonstrate that learning our semi-optimal policy ensures stable and high performance regardless of the size of $N$ and $T$.
Our code is available at https://github.com/isno0907/sosampler.

% To address this challenge, we introduce a novel perspective of prioritizing the reduction of search space complexity to ease its exploration. Discovering that the confidence scores from a fixed downstream classifier reasonably approximates the scores for the optimal combination of frames, we pose it as `semi-optimal policy', significantly reducing the search space complexity to $O(T)$. 

% Upon this, we propose the semi-optimal sampler (SOSampler), a lightweight framework that leverages single-frame confidence as pseudo-labels. SOSampler enables smaller networks to approximate the semi-optimal policy, offering a practical solution to the challenge of frame sampling even for the large $T$ and $N$. Through extensive experiments on multiple datasets, we demonstrate that our proposed method achieves the state-of-the-art.
\end{abstract}



%Frame sampling in video classification poses a significant challenge due to the computational impracticality of brute force searches across the combinatorial explosion of frame sets. To explore the search space, recent methods use reinforcement learning or sampling techniques, but these approaches struggle with increasing complexity as the number of frames grows, hindering efficient training. 
%Addressing this, we introduce a novel perspective inspired by knowledge distillation principles: prioritizing the reduction of search space complexity over final accuracy to ease computational load and optimization challenges.
%Our approach centers on the development of the 'Semi-optimal policy', a single frame clip confidence-informed sampling strategy. This method leverages the confidence output of a fixed downstream classifier, significantly reducing spatial complexity from $O(T^N)$ to $O(T)$. 
%Furthermore, we introduce the Knowledge Distillation Sampler (KDSampler), a lightweight framework that leverages single-frame confidence as pseudo labels.
%We analyze how optimal the proposed semi-optimal policy is and conduct extensive experiments on four benchmark datasets and four backbone architectures, demonstrating that our proposed KDSampler outperforms most existing state-of-the-art methods.




% Researches in action recognition have shown significant progress recently. However, the inherent challenges with digital videos like temporal redundancy and noise issues make video models inefficiently use computational resources. To address this problem, recent methods introduce frame sampler, which allows the pretrained classifier to focus on a smaller set of relevant frames, enhancing its effectiveness and efficiency. 
% Most of these methods, however, are highly approximate, relying on sampling techniques or reinforcement learning, instead of directly training a sampler in a supervised manner.
%However, there is currently no method to directly train a sampler without using sampling techniques or RL-based methods. And 
% Furthermore, these researches limit their scope to CNN architecture and do not translate properly to Transformer architecture. Motivated by these issues, we explore an optimal sampling policy that is not restricted by model architecture and investigate methods for directly approximating importance score for each frame. In this paper, we present KDSampler, a lightweight sampler that distills the sampling policy of confidence-based sampler, which quantifies the importance of each frame from downstream task performance. 
% \junho{The sampling problem is a combinational problem of finding the optimal combination within a given set of candidates. As it requires too much computational cost to find the optimal combination,
% by inferring every combination through a classifier, 
% previous methods have relied on sampling techniques or reinforcement learning. 
% However, if the optimal combination could be found within a reasonable time, it would be better to learn optimal sampling policy.
% Although these methods demonstrate impressive performance, there has been a lack of exploration into how the optimal sampling policy is determined based on the classifier, and whether there are any similar sampling policies.}
% \junho{In this paper, we introduce a confidence-based sampler that is based on the confidence of each frame and simulates an optimal sampler with a similar sampling policy. Furthermore, we propose KDSampler, a method that trains a light-weight network through knowledge distillation, enabling it to efficiently mimic confidence-based sampler.}
% In this end, we propose a confidence-based sampling approach, which samples based on the confidence of each frame in the classifier, and KDSampler, a method where this information is distilled into a light-weight sampler.
% \junho{From this perspective, we propose confidence-based sampling, which approximates the optimal sampling policy through the confidence of a pretrained classifier, and introduce KDSampler, a lightweight sampler that distills the sampling policy of confidence-based sampler.}


==> arXiv-2409.05260v4/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
As video platforms continue to grow explosively, efficient and scalable video understanding becomes increasingly important.
With remarkable advances in deep learning, action recognition and video understanding have also made tremendous progress, from 2D~\cite{ng2015snippets,fernando2016rankpooling,zhou2018trn, simonyan2014twostream,feichtenhofer2016twostreamfusion,lee2018cdml,lee2020gcml} and 3D CNN models \cite{tran2015c3d,carreira2017i3d,qiu2017p3d, tran2018r2+1d,feichtenhofer2019slowfast,tran2019csn} to Transformers \cite{arnab2021vivit,bertasius2021timesformer,liu2022videoswin}.
Despite these advances, video understanding models are still often overwhelmed by high storage and computational cost.
To mitigate this, lighter models with less parameters and computational cost \cite{zolfaghari2018eco,kopuklu2019resource,fan2019moreisless,feichtenhofer2020x3d,verelst2020dynamic,piergiovanni2022tvn} have been proposed.


Focusing mostly on the modeling aspect, however, these works have not touched the most basic underlying condition that digital videos are encoded as a temporal sequence of regularly sampled frames, where each frame is a 2D spatial matrix of regularly sampled pixels, regardless of the content.
These regularly sampled pixels are often highly redundant, especially when the frame rate is high.
Ideally, it will be more efficient to sample frames proportional to the amount of information, removing redundancy among them as much as possible.
Given that most existing video models are still built on a constant frame sampling rate for all videos, there are further room for improvement in terms of efficiency.

In this paper, we consider the frame sampling problem. For a video with $T$ frames, we propose a frame sampler that selects $N \ll T$ frames, which are then used by a video model pre-trained for a specific downstream task (e.g., classification).
%, so as to maximize the downstream task performance with the selected frames only.
The goal of this task is to train a sampler that finds the best combination of $N$ frames out of the given $T$ frames, letting the pre-trained model (classifier) to achieve the highest downstream task performance.

% 이걸 달성하기 위해 sampler는 T장의 frame이 주어졌을 때 가장 좋은 N장을 고르는 방법을 배워야 하고, 이걸 policy 라고 부른다.
% 가장 이상적인 policy는 (unseen test set에서) 최고의 downstream task performance를 내는 조합을 찾아주는 policy이고, 우린 이걸 Optimal policy라고 부르겠다.
To achieve this, the sampler learns a \emph{policy} to select $N$ frames out of $T$ candidates.
The ideal policy would select the best $N$ frames that lead to the highest downstream task performance, and we call this \emph{optimal policy} ($\pi_o$).
A naive approach would collect the best combinations as training data and train the sampler in a supervised manner.
%A naive approach in deep learning is to find the best combination for each video and use it as a label to train the sampler in a supervised manner.
However, finding the best combination is an NP-hard combinatorial optimization problem, as it requires comparing all $\binom{T}{N}$ possible combinations to find the solution.
Exhaustively searching this $O(T^N)$ space is practically infeasible when $N$ and $T$ grow.
%Since there are $\binom{T}{N}$ possible combinations of $N$ frames, however, the search space complexity is indeed $O(T^N)$, and exhaustive search of this space is practically infeasible.}

% A typical supervised learning setup would collect samples from this $\pi_o$ to train the sampler, and it reasonably works for small $N$ and $T$. \red{[CITE]}
% T장 중 N장을 뽑는 모든 조합은 O(T^N)만큼 존재하기 때문에, Optimal policy를 구하려면 이만큼의 space를 search해야 한다.
% 기존의 방법은 RL을 쓰거나 ~~ 해서 이 space를 탐색하지만, 본질적인 search space complexity는 바뀌지 않는다.
% \joonseok{Since there are $\binom{T}{N}$ possible combinations of $N$ frames, however, the search space complexity is indeed $O(T^N)$, and exhaustive search of this space is an NP-hard combinatorial problem.}
Several previous works~\cite{wu2019adaframe,wang2022adafocus,lin2022ocsampler,li2021ada2d,wu2019marl} have applied reinforcement learning to search this space, setting up the sampler as an agent and the classifier as the environment and training the sampler with a reward function designed to find $\pi_o$.
While they have shown promising results for small $N$ and $T$, the underlying search space of $O(T^N)$ still remains the same, posing challenges for large $N$ and $T$.
% making it less feasible with large $T$ and $N$.

%T, N이 커지면 계산량이 급증하거나, 계산량을 적게 유지할 경우 search space를 충분히 보지 못해 성능이 하락하는 문제가 생긴다.

%To achieve this, the sampler needs to learn an optimal policy ($\pi_o$) for finding the best combination. A naive approach in deep learning is to find the best combination (label) for each video instance and use it as a label to train the sampler in a supervised manner. However, finding the optimal combination is an NP-hard combinatorial problem, as it requires comparing all combinations to find the solution, making it practically infeasible.

%\red{Previous research~\cite{wu2019adaframe,wang2022adafocus,lin2022ocsampler,li2021ada2d,wu2019marl} has addressed this challenge by setting up the sampler as an agent and the classifier as the environment, designing a reward function, and training the sampler through sampling techniques to learn $\pi_o$.}

Considering the purpose of the frame sampling task, however, it is more important for the sampler to operate effectively on a long video with a large $N$ and $T$.
Unlike the previous works that operate directly within the $O(T^N)$ space, we take a step back to find a way to reduce this search space itself.
The fundamental reason for this exponential growth of search space is that the value of a selected frame depends on those of other selected frames and thus we need to consider the joint distribution of the frame values.

What if, however, the value of a frame can be fairly determined independently from each other?
We would be able to score $T$ frames independently and simply to take the top $N$ frames.
In this paper, we argue that, based on experimental results, frames can be reasonably assessed independently under most practical conditions where frame sampling is relevant—namely, when the video is not excessively short and the frame rate is not extremely high. We observe that a policy based on evaluating the value of each frame can reasonably approximate an optimal sampling policy.

% In this paper, we first claim that frames can be indeed scored independently under most practical settings that frame sampling does matter; that is, when the video is not trivially short and the frame rate is not extremely high.
Based on this observation, we propose a \textit{semi-optimal policy} ($\pi_s$) that selects the top $N$ frames based on estimated value of each frame using per-frame confidence.
This approach significantly reduces the search space to $O(T)$.
%Unlike the $\pi_o$ method, which examines all $\binom{T}{N}$ combinations to find the best performance, $\pi_s$ approximates the value of each frame using per-frame confidence scores, measured by feeding each frame as a single-frame video, and selects the top $N$ frames.
We empirically show on multiple datasets that $\pi_s$ is a policy that reasonably approximates $\pi_o$, and demonstrate that the state-of-the-art sampler~\cite{lin2022ocsampler} achieves more stable and superior performance when it learns $\pi_s$ instead of $\pi_o$, not only with small but also large $N$ and $T$.
%we demonstrate that our Semi-Optimal sampler (SOSampler), with the same structure as the existing SOTA sampler, learns $\pi_s$ instead of $\pi_o$, achieving more stable and higher performance not only for small $T$ and $N$ but also for large $T$ and $N$.

%The reason we face optimization challenges is that when $N \ll T$, the search space for finding the optimal solution becomes $O(T^N)$. This exponential increase in search space for $N$ occurs because the value of the selected frame depends on the other selected frame, and it is difficult to know how they affect each other without investigating all combinations. However, if the value of each frame is determined independently, we can solve the problem much more easily by evaluating the value of each frame and selecting the top $N$ frames.

%In this paper, based on the frame independent assumption, 


% The ultimate goal of frame sampling is to find the combination of $N$ frames that enables the classifier to best perform on the downstream task, from the $\binom{T}{N}$ possible sets.
% The most naive and straightforward approach is the brute force search of all possible combinations, incurring obviously impractical time complexity of $O(T^N)$.
% To explore this huge space, reinforcement learning~\cite{wu2019adaframe,wang2022adafocus,lin2022ocsampler,li2021ada2d,wu2019marl} or sampling techniques~\cite{wu2019liteeval,meng2020arnet,sun2021videoiq,meng2021adafuse} have been adopted.
% Without breaking the combinatorial optimization nature of the $O(T^N)$ space, however, these approaches suffer when $N$ becomes large.
% Sequential sampling~\cite{wu2019adaframe,wu2019liteeval, wang2022adafocus,meng2021adafuse,ghodrati2021frameexit,seon2023stoporforward} introduces a greedy decision process to select the next frame based on the down-stream task performance using previously selected ones, reducing the complexity to $O(NT)$.
% In spite of their light-weight sampling policy, however, they have an inherent limitation that the entire process needs to be repeated until the stopping condition is met, without taking advantage of parallelism.

% Thereby, we aim to reduce the search space, but at the same time to avoid sequential selection of each frame.
% Instead of designing a method better exploring the search space of $O(T^N)$ by precisely scoring each set of frames, we aim to shift our focus to reduce the search space, thereby lowering both computational load and optimization difficulty, at the cost of final accuracy.
% In other words, if the globally optimal selection of $N$ frames is considered as ground truth, our goal is to find a \emph{Semi-optimal} sampling policy with a significantly smaller search space, and to use it as a pseudo-ground-truth.

% To find a Semi-optimal sampling policy, we pay attention to a practical environment that the candidate frames convey sufficiently different information.
% (If most frames are almost identical, sampling any $N$ frames will lead to similar performance.)
% Under this setting, we empirically discover that the per-frame confidence score of the fixed classifier, measured by feeding each frame as a single-frame video, reasonably approximates the optimal set-level score of $N$ frames (see \cref{sec:semi} for more justification).
% This approach ignores interactions between frames, taking only $O(T)$ to score all frames, and thus we take it as our Semi-optimal sampling policy.
% This choice is somewhat analogous to the Naive Bayes, where each element is assumed to be independent of each other in spite of obvious violation, but practically performs reasonably.

% Based upon this cost-effective Semi-optimal sampling policy, we propose a Knowledge Distillation Sampler (KDSampler) that trains a light-weight sampler by distilling the Semi-optimal sampling policy as the teacher.
% In general, a student model that is trained on the prediction by a larger teacher model as a pseudo-label tends to outperform the same model trained solely on the ground truth label, since the pseudo-label presents more information (\emph{i.e.}, confidence scores) by the teacher, even if it is imperfect.
% Taking this advantage of knowledge distillation, our KDSampler learns to approximate Semi-optimal frame scores, with significantly smaller search space of $O(T)$.
%allows the light-weight network to approximate the proposed Semi-optimal policy using single frame confidence as a pseudo-label.

%On the other hand, parallel sampling methods~\cite{korbar2019scsampler,meng2020arnet} process all candidate frames at once.
%Thanks to the benefits from parallelism, both accuracy and efficiency of sampling has been improved.

%\junho{In knowledge distillation, training smaller network using the outputs of a pretrained larger model as pseudo-labels results in better performance than training smaller network with ground truth.
%One reason for this is that pseudo-labels, although less accurate than the ground truth, present information that is easier for the model to learn from, thereby reducing the difficulty of optimization. Inspired by this,}
%we aim to shift our focus from finding methods that optimize better across the entire search space to those that, even at the cost of final accuracy, reduce the search space, thereby lowering both computational load and optimization difficulty.
%In other words, if the optimal sampling policy is considered ground truth, our goal is to find sub-optimal sampling policies with smaller search spaces and propose them as pseudo-labels.

%In the process of finding a sub-optimal sampling policy, we pay attention to the fact that the downstream model (classifier) remains fixed.
%Based on this, we propose a single frame clip confidence-informed sampling policy called ``Semi-optimal policy". Semi-optimal policy is a method of sampling frames by considering the confidence output of the video classifier for a video clip composed of a single frame as an important score.
%This sampling policy reduces the spatial complexity to $O(T)$ because the importance score of one frame is not affected by others.
%We verify through experiments that Semi-optimal policy reasonably approximates the optimal sampling. 


Our contributions are summarized as follows:
\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \item We introduce a novel perspective of \textit{reducing the search space from $O(T^N)$ to $O(T)$} in frame sampling for video classification, proposing the semi-optimal policy.
    %\item {We introduce a novel perspective of reducing the search space in frame sampling for video classification, proposing semi-optimal policy that remarkably simplifies the search space from $O(T^N)$ to $O(T)$.}
    \item {Through various analyses, we demonstrate that the semi-optimal policy approximates the optimal policy \textit{under the most practical settings}.}
    \item {From extensive experiments, we show that a sampler learning the semi-optimal policy achieves stable and high performance across both small and large values of $N$ and $T$.}
    % \item {We introduce KDSampler, a lightweight network distilled to approximate semi-optimal policy using single frame confidence as pseudo-labels.}
    %\item \junho{We introduce a new perspective in parallel frame sampling for video classification, shifting from a focus on optimizing across a vast search space to developing sub-optimal sampling policies that significantly reduce the search space and computational load.}
    %\item \junho{We propose the Semi-optimal policy, a novel sampling policy that remarkably simplifies the spatial complexity from $O(T^N)$ to $O(T)$, offering a practical solution to the combinatorial challenge in frame sampling.}
    %\item \junho{We introduce the KDSampler, a tool that enables a lightweight network to approximate the Semi-optimal policy using single frame confidence as pseudo labels. This method leverages the principles of knowledge distillation, utilizing the outputs of a more complex model to enhance the performance of a simpler model.}
    % \item The proposed method achieves linear time and space complexity to the number of input frames, $O(T)$, as opposed to the exponential complexity of $O(T^N)$ where $N$ is the number of target frames to select with existing methods.
    % \item From extensive experiments, we demonstrate that the Semi-optimal policy effectively approximates the optimal sampling policy and that our KDSampler achieves the state-of-the-art.
\end{itemize}






==> arXiv-2409.05260v4/sec/2_relworks.tex <==
\section{Related Work}
\label{sec:related}

% \noindent
% \textbf{Video Recognition.}
% 2D and 3D convolutional neural networks (CNNs) have been widely used for image and video classification.
% %Video recognition methods can be broadly classified into 2D-CNN approaches and 3D-CNN approaches.
% 2D-CNN approaches apply 2D convolution filters along the spatial dimension for each frame, then aggregating them by feature pooling~\cite{ng2015snippets}, rank pooling~\cite{fernando2016rankpooling}, or relation network~\cite{zhou2018trn} to encode the temporal information of videos.
% Two-stream methods take both spatial stream from CNN and temporal stream from optical flow as input at various levels of fusion~\cite{simonyan2014twostream,feichtenhofer2016twostreamfusion}.

% 3D-CNN approaches apply convolution operations on both spatial and temporal dimensions simultaneously, pioneered by C3D~\cite{tran2015c3d}.
% I3D~\cite{carreira2017i3d} builds upon the 3D convolution and applies similar Inception modules used for 2D image classifications.
% P3D~\cite{qiu2017p3d} and R(2+1)D~\cite{tran2018r2+1d} show that factorizing the spatial and temporal dimensions in the 3D convolution results in higher performance.
% SlowFast~\cite{feichtenhofer2019slowfast} model consists of two different pathways of focusing more on temporal and spatial information, connected with lateral connections.
% CSN~\cite{tran2019csn} shows that separating the channel interaction with spatio-temporal interaction leads to lower computational cost and better regularization.

% More recently, Transformers~\cite{vaswani2017attention} have been used for video classification tasks (\emph{e.g.}, action recognition), developing convolution-free methods that rely on self-attention over spatial and temporal axes.
% As computational costs are high to process all patches in the video, most video Transformer models introduce methods to factorize spatial and temporal attentions~\cite{arnab2021vivit,bertasius2021timesformer} or to utilize the inductive bias of locality in videos \cite{liu2022videoswin} for efficient handling of videos.
\noindent
\textbf{Video Recognition.}
2D and 3D convolutional neural networks (CNNs) have been widely used for image and video classification.
2D-CNN encodes each frame individually, then aggregates the temporal dynamics by feature pooling~\cite{ng2015snippets,lee2018yt8m2,hwang2019video}, rank pooling~\cite{fernando2016rankpooling}, or relation network~\cite{zhou2018trn}.
%2D-CNN approaches apply 2D convolution filters along the spatial dimension for each frame, then aggregate them by feature pooling~\cite{ng2015snippets}, rank pooling~\cite{fernando2016rankpooling}, or relation network~\cite{zhou2018trn} to encode the temporal information of videos.
Two-stream methods take both spatial stream from CNN and temporal stream from optical flow as input at various levels of fusion~\cite{simonyan2014twostream,feichtenhofer2016twostreamfusion}.
3D-CNN approaches apply convolution operations on both spatial and temporal dimensions simultaneously, pioneered by C3D~\cite{tran2015c3d}.
I3D~\cite{carreira2017i3d} combines the 3D convolution with two-stream approaches.
P3D~\cite{qiu2017p3d} and R(2+1)D~\cite{tran2018r2+1d} factorizes the spatial and temporal dimensions in the 3D convolution.
SlowFast~\cite{feichtenhofer2019slowfast} model consists of two different pathways of focusing more on temporal and spatial information, respectively.
CSN~\cite{tran2019csn} shows that separating the channel interaction with spatio-temporal interaction leads to lower computational cost and better regularization.

Recently, Transformers~\cite{vaswani2017attention} have been applied to video classification and action recognition.
Due to the high computational cost for processing all patches in the video, most video Transformer models factorize spatial and temporal attentions~\cite{arnab2021vivit,bertasius2021timesformer} or utilize the inductive bias of locality in videos \cite{liu2022videoswin} for efficient handling of videos.


\vspace{0.1cm} \noindent
\textbf{Efficient Video Recognition.}
One of the biggest challenges of video classification is the computational cost stemming from the vast number of frames.
One remedy is to lighten the model architecture itself~\cite{zolfaghari2018eco,kopuklu2019resource,fan2019moreisless,feichtenhofer2020x3d,verelst2020dynamic,piergiovanni2022tvn}.
%Researches in this area can be largely divided into two categories of approaches. Firstly, there are approaches that propose novel algorithmic structures based on pre-trained backbones and sampling policy to achieve performance enhancement efficiently.
Another direction is algorithmic improvement for better efficiency.
AdaFrame~\cite{wu2019adaframe}
% employs an LSTM-based agent that
learns from both the current frame and the global context to make decisions on where to look next in the video.
AdaFocus series~\cite{wang2022adafocus, wang2021adafocus} use a lightweight global CNN to guide the policy network to extract the most useful image crop to classify the video.
On-the-fly gating techniques are introduced to reduce computation by only extracting finer features at selected frames~\cite{wu2019liteeval}, determining an early exiting point~\cite{ghodrati2021frameexit}, or deciding which frames in the video to fully process~\cite{seon2023stoporforward}. ListenToLook~\cite{gao2020listentolook} utilizes only a single frame and audio stream to determine the full video descriptor for the clip.


An alternative is to sample frames to process, instead of feeding all of them to the classification model, vastly reducing the computational cost.
%Instead of changing the model architecture itself, an efficient sampling method vastly reduces the computing cost by using only a subset of frames that can still accurately predict video information.
%Secondly, there are techniques that aim to improve performance by selecting optimal frames to maximize the performance of trained classifiers through samplers. 
ARNet~\cite{meng2020arnet} and VideoIQ~\cite{sun2021videoiq} pre-train multiple classifiers and train a sampler to determine which classifier to process each frame. MARL~\cite{wu2019marl} utilizes multiple agents that adjust the sampling location based on local and historical context. OCSampler~\cite{lin2022ocsampler} simply selects the salient frames, while Ada2D~\cite{li2021ada2d} determines which frames will be used in 2D or 3D.
Ours falls into this category, particularly aiming to effectively sample $N$ frames for a large $T$.

% Researches in this area can be largely divided into sequential and paralleling methods.
% Sequential sampling methods select the frames sequentially, relying on the previously selected frames to decide whether to sample more frames or to stop the procedure.
% AdaFrame~\cite{wu2019adaframe} relies on LSTM-based agent that learns from both the current frame and the global context to make decisions on where to look next in the video.
% AdaFocus~\cite{wang2022adafocus} uses a lightweight global CNN to guide the policy network to extract the most useful crop of the image to classify the video.
% On-the-fly gating techniques are introduced to reduce computation by only extracting finer features at selected frames \cite{wu2019liteeval}, determining an early exiting point \cite{ghodrati2021frameexit}, or deciding which frames in the video to fully process~\cite{seon2023stoporforward}. 

% In parallel sampling methods, the selection of frames is processed in parallel, without the need for information from other frames. 
% SCSampler~\cite{korbar2019scsampler} trains a clip-level saliency model with a cross entropy as a loss to determine which clips are most important in classifying the video.
% ListenToLook~\cite{gao2020listentolook} utilizes only a single frame and audio stream to determine the full video descriptor for the clip.
% MARL~\cite{wu2019marl} uses multiple agents that adjust the sampling location from local and historical context.
% Other methods commonly learn a policy that determines which frames to select \cite{meng2020arnet,sun2021videoiq,li2021ada2d,lin2022ocsampler}, while further utilizing the policy to determine resolution to process the frames at \cite{meng2020arnet}, bit-width for processing the frames \cite{sun2021videoiq}, or which 3D convolution to keep or discard \cite{li2021ada2d}.
% MGSampler~\cite{zhi2021mgsampler} preprocesses the video by capturing the motion in the video.

% In both branches of methods, sampling techniques (\emph{e.g.} gumbel softmax or RL) are widely used to train the sampler.


% \vspace{0.1cm} \noindent
% \textbf{Ranking loss.}
% %\junho{
% Ranking loss is widely used for tasks to learn relative relevance between two or more objects, such as recommendation systems. The underlying idea behind the ranking loss is to model the relative order of preference between pairs of items rather than predicting their absolute labels.
% %It can reduce the effort that will be used to learn useless information about ordering.
% In the context of video frame sampling, SCSampler \cite{korbar2019scsampler} has tried to apply ranking loss as an additional loss to train its saliency model, but they reported the ranking loss rather exacerbated the performance.
% In this paper, we carefully adapt this idea to our SOSampler, successfully improving the overall performance.


% \input{figures/overview}

==> arXiv-2409.05260v4/sec/3_method.tex <==
\section{Problem Formulation}
\label{sec:problem}

\noindent
\textbf{Sampling Scenario.}
We assume an offline environment, where we are given $T$ candidate frames $\bm{v} \in \mathbb{R}^{T \times 3 \times H \times W}$ from a video, with $H$ and $W$ indicating the height and width of the frames, respectively.
% where $H$ and $W$ indicate the height and width of the frames, respectively.
A frozen pretrained classifier $f_c: \mathbb{R}^{N \times 3 \times H \times W} \rightarrow [0,1]^{C}$ is given, where $N$ is the number of input frames and $C$ is the number of classes.
In this context, our final objective is to train a sampler that finds the optimal $N$ frames out of the given $T$ frames that make the classifier to best perform on the downstream task.

\vspace{0.1cm}
\noindent\textbf{Optimal Policy $\bm{\pi_o}$.}
Given $T$ candidate frames, the optimal policy $\pi_o$ chooses $N$ frames that maximize the confidence of the classifier $f_c$ on the true label $y \in [1, ..., C]$, among all possible combinations of the candidate frames. We define the frames selected by $\pi_o$ as optimal set.
% \red{$\pi_o$ is not practical as it relies on the true label, but we aim for our sampler to learn it.}
% Note that even with the optimal policy, the upperbound of the final performance depends on the pretrained classifier.

% Basically, a frame sampler aims to learn $\pi_o$. The most naive approach to learn $\pi_o$ is that firstly we find the optimal set of each video and train the sampler to find the optimal set among the candidate frames in supervised manner. However, finding the optimal set is combinatorial optimization problem, which is NP-hard, so we need to exhaustively try every possible combinations with $O(T^N)$ search space. Even for slightly large $T$ and $N$, search space becomes vast and makes it challenging for a sampler to directly be trained. 

\vspace{0.1cm}
\noindent\textbf{Challenges.}
% The most straightforward approach to learn $\pi_o$ would be to \joonseok{train a sampler in supervised manner to select the best set of frames, exhaustively discovered for the training videos.}
The most straightforward approach to learn $\pi_o$ would be to train a sampler in a supervised manner to select the optimal set of frames.
% first identify the optimal set for each video %\joonseok{in the training dataset} and then train the sampler to select the optimal set among the candidate frames in a supervised manner.
% \joonseok{However, exhaustively searching for the optimal set of frames is computationally prohibitive, requiring to explore a search space of $O(T^N)$.}
However, finding the optimal set of frames is computationally prohibitive, requiring to explore a search space of $O(T^N)$.
% However, finding the optimal set is combinatorial optimization problem, which is NP-hard, so we need to exhaustively try every possible combinations with $O(T^N)$ search space.
Even for moderately large $N$ and $T$, the search space quickly grows, making it challenging to train the sampler directly.

To explore this space, previous works adopt reinforcement learning, where a network sampler (agent) is trained based on rewards given by the classifier (environment) for the selected frames (action) according to the policy.
Although these approaches have been effective for small $N$ and $T$, they are not scalable for growing $N$ and $T$.
% they still face challenges when $T$ and $N$ are large.
To mitigate the exponential time complexity caused by this exponentially growing search space, we propose an effective approach in most practical settings.
% a somewhat crude-looking but in fact 
%\junho{We analyze that the exponential increase in the search space with respect to $N$ poses significant optimization challenges. Therefore, we aim to find the way to mitigate these optimization challenges.}
% While these approaches have effectively improved performance for small $T$ and $N$, they still struggle with large $T$ and $N$. We analyze that the exponential increase in the search space with respect to $N$ leads to significant optimization challenges. Therefore, we aim to find methods to alleviate this optimization challenges.
% However, these approaches have limitations, as the combinatorial optimization problem leads to an exponentially increasing search space as $N$ grows, making them effective only for small $N$.

% As the frame sampling task is a kind of combinatorial problem and combinatorial problem is NP-hard problem which has $O(T^N)$ search space. Because the search space exponentially increases as $N$ grows, it is hard to optimize the sampler. So previous works only do their experiment on small $T$ and $N$.
% , prohibitively expensive to implement in practice, especially when $N$ gets high.

%--------------------------------------------------
%\vspace{0.1cm}
\section{Method}
\label{sec:method}
\subsection{Semi-Optimal Policy}
\label{subsec:semi}
% In this section, we propose a novel, approximately optimal sampling policy, which aims to resolve this issue by significantly reducing the complexity of search space.
%finding a sub-optimal policy that reduces spatial complexity.
% \junho{In this section, we present the assumption we suggest to alleviate the optimization challenge and the experimental result that support this assumption. Based on this, we propose a new sampling policy that effectively approximates the sampling policy of $\pi_o$ while significantly reducing the space complexity to $O(T)$.}
The main challenge of the frame sampling problem lies in the fact that the importance of a frame is influenced by other selected frames, necessitating to explore the interactions in the exponentially growing search space to $N$ and $T$.
% \joonseok{Strictly speaking, the importance of any selected frame is influenced by other selected ones, and it causes the exponential growth of the search space, necessitating the exploration of all combinations.}
%\junho{The frame sampling problem is challenging to solve because the importance of any selected frame is influenced by other selected frames, necessitating the exploration of all combinations with large search space.}
%The reason the frame sampling problem is challenging to solve is that the importance of any selected frame is influenced by other selected frames, necessitating the exploration of all combinations.
% \joonseok{Conversely, we take our attention that the problem would be much simpler 1) if the importance of each frame is (roughly) independent of other frames and 2) if we can reasonably approximate the importance of each frame, allowing us to simply scoring $T$ frames individually and to select the top $N$ out of them.}
Conversely, we recognize that the problem would be much simpler if: 1) the importance of each frame were (roughly) independent from other frames, and 2) we could reasonably approximate the importance of each frame.
This would allow us to score $T$ frames individually and select the top $N$ of them.
%However, if we satisfy two conditions: 1) the importance of each frame is independent of other frames, and 2) we can score this importance, the problem becomes much simpler.
%\junho{By scoring the importance of each frame and selecting the top $N$ frames, the search space reduces to $O(T)$.}
%frame sampling의 practical setting에서 프레임들 사이의 독립성을 분석하고

In this section, we show that the frames are indeed close to independence when it comes to a practical setting of the frame sampling task -- where the video is not trivially short and the frame rate is relatively low.
The opposite case, a short snippet with high frame rate, would not need a sophisticated frame sampling method anyway,
%benefit from frame sampling anyway,
since most frames would be highly redundant.
From this observation,
we introduce a new sampling policy that effectively approximates the optimal policy while significantly reducing the space complexity.

%\junho{In this section, we analyze the independence between frames in the practical setting of the frame sampling task and propose a method to score the importance of each frame.
%Based on these analyses, we introduce a new sampling policy that effectively approximates the optimal policy while significantly reducing the space complexity.}

% \subsection{Theoretical Justification}
% 우리는 프레임들이 서로의 가치에 영향을 끼치는 원인이 겹치는 정보에서 발생한다고 주장한다. 즉 아무리 중요한 정보를 가진 프레임이라도 다른 프레임들에서 이미 제공 중이라면 새로운 측면의 정보를 제공하는 프레임의 가치보다 떨어지게 된다. 그리고 여기서 새로운 정보라는 것은 비슷한 두 프레임보다 다른 프레임에서 발생하기 쉽다. 따라서 프레임들 간에 서로 다름이 보장될 수록 프레임끼리 정보가 겹칠 우려가 적어지고 각 프레임의 가치를 독립적으로 결정할 수 있게 된다.
% 따라서 frame per second (FPS)에 따른 프레임 간의 유사도를 조사하여 프레임 가치의 독립성을 분석해보고자 한다.
\vspace{0.1cm} \noindent
\textbf{Independence between Frames.}
% \subsection{Independence between Frames}
We claim that frames influence each other's importance mainly due to the overlapping information between them.
That is, even if a frame contains important information, its importance will be diminished if the same information is redundantly provided by others.
Conversely, the importance of a frame increases if it contains accurate and unique information; in other words, if it provides distinct information that is not covered by other frames.
%Here, "new information" is more likely to be found in frames that are dissimilar from one another.
Thus, if a candidate frame is sufficiently dissimilar from others, we would be able to independently score it without concerning redundancy.
%\junho{Thus, as the guarantee of dissimilarity between candidate frames increases, the concern of overlapping information between frames decreases, enabling us to independently determine the importance of each frame.}

To check applicability of this idea, we measure the similarity between adjacent frames at various frame rates.
%\junho{Therefore, we aim to analyze the independence of frame importances by investigating the similarity between frames based on frames per second (FPS).}
The similarity can be computed in several resolutions; as coarse as the probability distribution over the class labels, or as fine-grained as the pixel-level.
Both extremes are less ideal, since they do not convey high-level semantics of each frame.
Thus, we estimate the relevance between two sampled frames $i$ and $j$ by applying a Gaussian smoothing kernel to their visual embeddings, denoted by $\mathbf{x}_i$ and $\mathbf{x}_j$:
%Thus, we use their visual embeddings, $\mathbf{x}_i$ and $\mathbf{x}_j$, applying a Gaussian kernel to estimate the relevance between two sampled frames $i$ and $j$: %estimate the joint distribution by
\begin{equation}
  \mathcal{I}(\mathbf{x}_i, \mathbf{x}_j) = %\propto 
  \frac{1}{Z} e^{\left\{ -\frac{1}{2} (\mathbf{x}_i - \mathbf{x}_j)^\top \Sigma^{-1} (\mathbf{x}_i - \mathbf{x}_j) \right\}}, 
  % \nonumber
\end{equation}
where $\Sigma$ determines the kernel bandwidth and $Z = 1/|\sqrt{2\pi \Sigma}|$ is the normalizer.

% We claim that the relationship between frames comes from the information overlap about the label. For instance, if there are two frames, $\bm{v}_1$ and $\bm{v}_2$, that closely resemble each other and contain a lot of label information, and another frame, $\bm{v}_3$, with relatively less information but containing new label information, when $\bm{v}_1$ is selected, the value of $\bm{v}_3$ becomes higher than that of $\bm{v}_2$. Therefore, if the similarity between candidate frames is sufficiently low, we can independently evaluate the value of each frame based solely on the information it contains.

% We aimed to evaluate the independence between frames by comparing the similarity of visual embeddings of frames sampled at various FPS.


\input{figures/mutual_infomation}


\cref{fig:mutual_info} illustrates the estimated relevance
%plot to estimate the similarity
between two consecutive frames at various frame rates on ActivityNet-v1.3, using ResNet50 and TimeSformer features.
We observe with both features that higher frame rates lead to higher redundancy between frames.
%With an increased frame rate, the redundancy between frames also increases, as observed with both features.
%The plots show that as the FPS increases, the similarity between features also increases for both ResNet50 and TimeSformer models.
Although this tendency is expected considering the nature of videos, what we need to focus is \emph{where is the proper frame rate threshold} that we can safely assume independence between frames.
%\junho{While this is an expected result considering the nature of videos, what we need to focus on is the FPS threshold at which the independence assumption between frames is valid.}
From the plots, we conclude that we can reliably assume independence up to 1 fps, while 5 fps is on the borderline.
%By analyzing the plots, we can see that up to FPS 1, we can reliably assume independence, and FPS 5 is borderline.
Under a practical setting for frame sampling, we claim that 1 fps is still reasonable, since higher frame rates would be prohibitively expensive for long videos; \emph{e.g.}, for a 5-min-long video, 5 fps already piles up 1,500 candidate frames.
In short, we can reasonably assume independence among frames when the target video is not trivially short, since we would only feed regularly sampled frames at lower frame rate due to the computational overhead.
%\junho{Considering the practical settings of candidate frames in long videos, the upper limit of FPS at 5 is generous. Therefore, we can support the independence assumption between frames in the frame sampling task.}

% When $\bm{v}_1$ and $\bm{v}_2$ are identical at pixel level, $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j) = 1$.
% For a slightly relaxed case, where the two frames are almost identical at pixel level ($\bm{v}_1 \approx \bm{v}_2$; \emph{e.g.}, two consecutive frames at 30 fps), we observe in \cref{fig:mutual_info}(a) that $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$ is high, with the mean of 0.86, reflecting their significantly overlapping information.
% %
% For two consecutive frames at 1 fps, which is closer to the experimental setting in \cref{sec:exp}, we see in \cref{fig:mutual_info}(b) that most pairs are almost independent, with the mean of $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j)$ around 0.07.
% This is an upper-bound within the candidate frames, since non-consecutive frames would depend less on each other.
% %
% \cref{fig:mutual_info}(c) shows two frames from different videos have $\mathcal{I}(\mathbf{x}_i, \mathbf{x}_j) = 0$ for most cases, indicating strong independence.

% {These empirical measurement strongly implies that a set of frames can be reasonably approximated by the sum of their individual scores, unless the candidate frames are temporally too close as in the case of 30 fps.}

%\red{These empirical measurement indicates that 1) our theoretical analysis is sufficiently practical, and 2) it explains why our proposed method performs well even though it relies on an assumption that looks implausible at a glance. That is, dependence between two frames is in most cases negligible, unless they are extremely close temporally.}

% 앞서 언급한 2가지 조건 중 프레임 독립조건이 만족된다면 나머지 하나인 중요도를 점수매길 수 있다면 우리는 문제를 쉽게 만들 수 있다. 이 조건은 아주 간단하게 해결될 수 있는데, 각 프레임을 single-frame으로 구성된 비디오 클립으로 여기고 pre-trained classifier를 통해 추론했을 때 나오는 confidence 값을 우리는 사용할 수 있다.
\input{figures/confidence_based_sampler}
\vspace{0.1cm} \noindent
\textbf{Semi-optimal Policy $\bm{\pi_s}$.}
% \subsection{Semi-optimal Policy $\bm{\pi_s}$}
% Based on this observation, we propose the Semi-optimal policy $\pi_s$, which operates under the assumption that the selection of any frame is not influenced by other frames.
% Specifically, $\pi_s$ measures the importance of each frame based on its confidence score and chooses the top $N$ frames with highest scores.
% Note that $\pi_s$ treats each candidate frame $\bm{v}_t \in \mathds{R}^{H \times W \times 3}$ as a single-frame video clip $\bm{v}_t \in \mathds{R}^{1 \times H \times W \times 3}$ (we slightly abuse the notation to unclutter).
% It infers the confidence scores for all classes, $f_c(\bm{v}_t) \in [0, 1]^C$ for $t = 1, ..., T$.
Under the frame independence condition,
% one of the two conditions mentioned earlier, is satisfied, and 
we score the importance of each frame independently.
%we can score the importance of the frames, we can simplify the problem.
Specifically, we infer the frame-level confidence scores for all $C$ classes by
%distribution
%This condition can be easily addressed with a slightly different approach called frame clip confidence distribution: 
treating each frame $\bm{v}_t \in \mathds{R}^{H \times W \times 3}$ as a single-frame video clip $\bm{v}_t \in \mathds{R}^{1 \times H \times W \times 3}$ and take its confidence scores $f_c(\bm{v}_t) \in [0, 1]^{C}$.
We illustrate the mechanism of $\pi_s$ in \cref{fig:confidence-based sampler}.

In order to score the importance of a frame, its confidence scores $f_c(\bm{v}_t)$ on $C$ classes need be aggregated into a single confidence score $c(\bm{v}_t) \in \mathds{R}$.
There are two options for this.
First, we may take the confidence for the true label $y$ as importance score.
That is, $c(\bm{v}_t) = [f_c(\bm{v}_t)]_y$, where $\left[ f_c(\bm{v}_t) \right]_y$ indicates the confidence of frame $\bm{v}_t$ for the label $y$ using the classifier $f_c$.
This approach aims to learn the desired importance score for the actual class.
The second option takes the maximal confidence across all classes $i = 1, ..., C$; that is, $c(\bm{v}_t) = \max_{i=1, ..., C} \left[ f_c(\bm{v}_t) \right]_i$.
% At a glance, this may not look optimal, since the maximal confidence is not necessarily for the true class.
Motivation of this approach is to train the sampler with more consistent scores, since the importance may significantly vary depending on the labels even for similar scenes.
%\junho{Sometimes, even for similar scenes, the importance scores can vary significantly depending on the video labels. This can confuse the sampler's learning process. 
%Therefore, this is a trick to train the sampler more effectively by providing consistent scoring, even if it is less accurate score.}
Once we have the frame-wise confidence distribution $c(\bm{v}_t)$ for $t = 1, ..., T$, we select the top $N$ frames with highest importance score. That is,
\begin{equation}
    \label{eq:conf-based}
    \pi_s(\bm{v}, y;N) = \operatorname*{top-\textit{N}}_{t = 1, ..., T} c(\bm{v}_t).
\end{equation}
% However, this approach is unavoidable at testing, as we do not know the true class.
% To better simulate the testing environment, we may train the classifier using the maximal confidence, even if it is not for the true class.
% Sometimes the importance score significantly changes as a video label even if it is a similar scene and it can make sampler confuse to learn.
% \red{As illustrated in~\cref{fig:confidence-based sampler}, }

% \input{tables/oracle_conf_perform}
% \input{tables/oracle_conf_indice}
\input{tables/oracle_conf_performance_fidelity}

\vspace{0.1cm} \noindent
\textbf{Empirical Verification.}
We verify that our proposed policy $\pi_s$ reasonably approximates the optimal policy $\pi_o$ in practice.
%We suggest that our proposed policy $\pi_s$ can reasonably be the substitution of optimal policy $\pi_o$.
First, we actually compare the frame sampling performance of $\pi_s$ against $\pi_o$ with two architectures, a CNN and a transformer, on two datasets, ActivityNet-v1.3~\cite{caba2015activitynet} and Mini-Kinetics~\cite{kay2017kinetics}, representing the untrimmed and trimmed video datasets, respectively.
% Note that, within each architecture, we use the exactly same weights and only vary the sampling policy.
\cref{tab:oracle_conf_sampler_result} compares the performance of a pre-trained classifier when it takes a set of $N=6$ frames selected from $T=10$ frames by various sampling policies:
%In \cref{tab:oracle_conf_sampler_result}, we report the performance of the classifier, depending on the different sampling policies of the 
uniform sampling ($\pi_u$), the optimal policy ($\pi_o$), our semi-optimal policy ($\pi_s$), and using all frames without sampling (All).
%Given $T=10$ candidate frames, each policy selects $N=6$ frames using their sampling policy. Note that classifiers are fixed and only the sampling policy is varied. 
The results indicate that $\pi_s$ demonstrates significant improvement over $\pi_u$ and `All' under all settings, most closely approximating the optimal policy, $\pi_o$.
% As a baseline, we adopt uniform policy $\pi_u$, which uniformly selects $N$ frames from each video.
% Both $\pi_o$ and $\pi_s$ sample $N$ frames based on their respective policies from $T$ candidate frames.
% \cref{tab:oracle_conf_sampler_result} shows that $\pi_s$ demonstrates significant improvements over $\pi_u$ and `All frames' under all settings, indicating $\pi_s$ effectively approximates $\pi_o$.
%\junho{when evalutating improvemnets from $\pi_u$, it is observed that $\pi_s$ exhibits lower performance gains compared to $\pi_o$. However, it still demonstrates significant improvements across all experiments. }

Additionally, we report the sampling fidelity, which indicates the similarity of the sampled set to the optimal set, across various values of $N$. 
% we assess the similarity between $\pi_s$ and $\pi_o$ by measuring the sampling fidelity, which represents the overlap ratio between the set sampled by $\pi_s$ and that by $\pi_o$.
Formally, sampling fidelity is defined as $\mathbb{E}_{\bm{v}}\left(|\mathcal{S}_t(\bm{v}) \cap \mathcal{S}_o(\bm{v})| / N \right)$, where $\mathcal{S}_t(\bm{v})$ and $\mathcal{S}_o(\bm{v})$ denote the sampled set of frames from the video $\bm{v}$ by the target policy ($\pi_t$) and $\pi_o$, respectively.
\cref{tab:fidelity} compares sampling fidelity of our $\pi_s$ against two baselines: the random sampling and a deterministic coarse-to-fine sampling policy proposed in FrameExit~\cite{ghodrati2021frameexit}.
%We set the random sampling and a deterministic coarse-to-fine sampling policy proposed in FrameExit~\cite{ghodrati2021frameexit} as baselines. 
%\cref{tab:fidelity} reports that,
We observe that our $\pi_s$ demonstrates significantly higher sampling fidelity than the FrameExit policy, which exhibits fidelity nearly identical to the random policy.
%Unlike the FrameExit policy, which exhibits fidelity nearly identical to the random policy, $\pi_s$ demonstrates significantly higher sampling fidelity to the oracle set in all cases.
We also provide a qualitative comparison in \cref{sec:success_case}--\ref{sec:failure_case}.
% that unlike the FrameExit policy which exhibits nearly identical to random policy, $\pi_s$ demonstrates a significantly higher sampling fidelity to the oracle set in all cases.
% We also conduct qualitative comparison in \cref{sec:success_case}--\ref{sec:failure_case}.


\vspace{-0.1cm}
%--------------------------------
\subsection{SOSampler: Semi-optimal Policy-based Sampler}
\label{sec:sosampler}

As shown in \cref{subsec:semi}, our semi-optimal policy $\pi_s$ reasonably approximates the optimal policy $\pi_o$.
To train a lightweight network sampler based on this policy,
%\junho{However, as mentioned in \cref{sec:problem}, our ultimate goal is to train a lightweight network sampler. Therefore, in this section,
we propose the Semi-Optimal Sampler (SOSampler), which learns $\pi_s$ instead of $\pi_o$ in a straightforward manner.
\vspace{0.1cm}
% \subsection{Overview} 
% \label{sec:sosampler:overview}
\input{figures/overview}
\noindent\textbf{Overview.}
\cref{fig:overview} illustrates an overview of our approach, which consists of a frame sampler $S_\text{SO}$ and an action classifier $f_c$.
At training, we first 
%randomly sample 
take $T$ candidate frames from the input video and compose a video clip $\bm{v}$.
The classifier $f_c$ takes each candidate frame as a single-frame clip input and conducts classification.
This process is performed individually for each frame, producing $T$ predictions in total.
%therefore we get $T$ predictions based on each frame.
From these $T$ predictions, we take the representative confidence $c(\bm{v}_t)$ either by taking the true label $y$ or by taking the maximal one, as explained in \cref{subsec:semi}.
We then apply softmax to get a normalized importance distribution $\bm{p}_s \in \mathds{R}^{T}$.
% $\bm{p}_s \in \mathds{R}^{T}$:
% \begin{equation}
%     \label{eq:importance_dist}
%     \bm{p}_s = \text{softmax} \left\{ c(\bm{v}_1), ..., c(\bm{v}_T) \right\}.
%     %\bm{p_s} = \left\{ [f_{c}(\bm{v}_1)]_{y^*}, ... , [f_{c}(\bm{v}_T)]_{y^*} \right\},
% \end{equation}
%where $y^*$ is the representative confidence score, either the true label ($y^* = y$) or the one with the maximal confidence score ($y^* = \max_{i=1, ..., C} [f_c(\bm{v}_t)]_i$ for $t = 1, ..., T$).
%\junho{In implementation, we use max confidence instead of label confidence because of inconsistency issue.}
Then, our sampler $S_\text{SO}$ takes the \emph{spatially down-sampled} version of the same $T$ candidate frames.
$S_\text{SO}$ predicts the importance scores $\bm{\hat{p}}_s \in \mathds{R}^{T}$ over them and classifies each frame into the $C$ classes using linear projections.
See \cref{sec:model} for more detailed description.

% \vspace{0.1cm}
% \subsection{Model Configuration}
% \label{sec:sosampler:model}
% \vspace{0.1cm} \noindent
% \textbf{Model Configuration.}


% \subsection{Training Objectives}
% \label{sec:method:training}
\vspace{0.1cm} 
\noindent\textbf{Training Objectives.}
% As shown in \cref{subsec:semi}, Semi-optimal policy $\pi_s$ reasonably approximates the oracle policy $\pi_o$.
% As our sampler $S_\text{so}$ reproduces the importance score $\bm{p}_s$ of $\pi_s$, we can sample the important frames based on this score.
% Therefore, we aim to train the sampler $S_\text{so}$ to distill the importance score information from $\pi_s$.
We train the sampler $S_\text{SO}$ with two objectives: 1) the semi-optimal policy loss $\mathcal{L}_\text{SO}$, penalizing when the estimated importance score $\bm{\hat{p}}_s$ does not agree with the confidence $\bm{p}_s$ produced by $f_c$, and 2) the label guidance loss $\mathcal{L}_\text{LG}$, penalizing when the predicted class of each frame differs from the true label to ensure that each frame contains information about the video-level class.
% 각 프레임에 feature가 비디오 클래스의 레이블에 대한 정보를 담게 하기 위해 각 프레임마다 추정한 class가 true label class와 다를 때 패널티를 주는 label guidance loss
% First, the knowledge distillation loss $\mathcal{L}_\text{so}$ minimizes the gap between the importance $\bm{\hat{p}}_s$ predicted by our sampler (Eq.~\eqref{eq:importance_prediction}) and the importance score $\bm{p}_s$ (Eq.~\eqref{eq:importance_dist}) by the classifier $f_c$.

For $\mathcal{L}_\text{SO}$, we initially experimented with mean square loss, $\| \bm{\hat{p}}_s - \bm{p}_s \|_2$, but the result was not satisfactory.
Taking inspiration that what we need is a correct ordering of the importance scores, not their exact values, we adopt a pairwise ranking loss~\cite{lee2014lcr} for  $\mathcal{L}_\text{SO}$, which penalizes the model when the relative order of importance between a pair of two frames is reversed:
\vspace{-0.07cm}
\begin{equation}
    \mathcal{L}_\text{SO} = \sum_{(p_i, p_j)\in \Psi}{\text{sign}(p_i - p_j) \cdot \text{max}\left( \gamma+\hat{p}_i - \hat{p}_j, 0\right)},
    \label{eq:ranking}
\end{equation}
where $\Psi = \{(p_i, p_j); p_i > p_j\}$, $\text{sign}(z)$ is the sign function, and $\gamma$ is a hyperparameter indicating a target margin. 
For $\mathcal{L}_\text{LG}$, we use the cross-entropy loss.
% \red{While the importance score $\bm{p}_s$ is obtained using the label information, the sampler $S_\text{SO}$ does not have access to the true label during training.
% To address this issue, we add a classification loss $\mathcal{L}_\text{LG}$ to train the classifier $h_c$, using the cross-entropy loss.}

The overall loss function is constructed by
\begin{equation}
    \label{eq:total_loss}
    \mathcal{L} = \lambda \cdot \mathcal{L}_\text{SO}(\bm{p}_s,\bm{\hat{p}}_s) + (1-\lambda) \cdot \mathcal{L}_\text{LG}(\bm{\hat{y}}_s, \bm{y}),
\end{equation}
where $\lambda$ is a hyperparameter that adjusts the ratio of the two losses, $\bm{\hat{y}}_s$ denotes the predicted confidence scores by the sampler and $\bm{y}$ is the one-hot encoding of the true label $y$.


\vspace{0.1cm} \noindent
\textbf{Inference.}
At inference, $T$ candidate frames are uniformly sampled from the target video.
%at uniform intervals.
As in training, each frame is down-sampled and fed into the sampler $S_\text{SO}$ to obtain the importance scores.
Frames with the top $N$ scores are selected, and those selected frames in the original resolution are fed into $f_c$ to perform the final classification.

% Below, we describe components of SOSampler in more details.


==> arXiv-2409.05260v4/sec/4_experiment.tex <==
\section{Experiment}
\label{sec:exp}


% \input{tables/timesformer}
\subsection{Experimental Setup}
\label{sec:exp:setup}

\noindent\textbf{Datasets.}
We evaluate on four public video classification benchmarks:
ActivityNet-v1.3~\cite{caba2015activitynet},
Mini-Kinetics~\cite{kay2017kinetics},
Mini-Sports1M~\cite{karpathy2014sport1m}, and 
COIN~\cite{coin}.
See \cref{sec:dataset} for more detailed description about the datasets.

% FCVID, comprising 239 action labels, contains 45,611 training videos and 45,612 validation videos with an average duration of 167 seconds. 

\vspace{0.1cm}
\noindent\textbf{Experimental Protocol.}
We randomly sample $T$ frames from each video as a training example and uniformly sample $T$ frames from each test video.
We use MobileNetv2TSM~\cite{sandler2018mobilenetv2,lin2019tsm} as the feature extractor of our sampler $S_{\text{SO}}$ and one additional fully-connected layer at the head of the sampler, following~\cite{lin2022ocsampler}.
See \cref{sec:implementation} for more details.
% for our experiment. 
% Firstly, $T$ frames are randomly sampled from video as a training example.
% All frames are randomly scaled and cropped to $224 \times 224$, followed by random flipping for augmentation.
%Then we randomly scale all frames and randomly crop $224\times224$ image patch, and apply random flipping for augmentation.
%apply random cropping to obtain frames with $224\times224$ resolution, while also randomly flipping the frames.
% We then reduce the resolution of each frame to $128 \times 128$ before feeding them into our sampler $S_\text{KD}$. 
% At inference, we uniformly sample $T$ frames from a test video, resize them to $128\times128$, and feed them to the sampler $S_\text{KD}$.
%During inference, we continue to use $128\times128$ resolution frames to feed $S$,
% Then, we feed the original $224 \times 224$ images of the selected frames to $f_c$.
%and for the sampled frame source, we perform a center cropping frame of size $224\times224$.

% In \cref{table:sota_actv_fcvid} and \cref{table:sota_sport_coin}, we conduct experiments with $T=10$ and $N=6$ following~\cite{lin2022ocsampler}. For the backbone of our sampler $S_\text{so}$, we use MobileNetv2TSM~\cite{sandler2018mobilenetv2,lin2019tsm}.
% On ActivityNet and Mini-kinetics datasets with the ResNet50 classifier, we use pre-trained weights provided by \cite{ghodrati2021frameexit}. And we train the classifier for the other dataset and architecture.
% And we train a TimeSformer classifier using 6 randomly sampled frames with size of $224\times224$ for all datasets.

% To train our SOSampler, we use learning rate of $10^{-3}$ and $\lambda = 0.99$ on all datasets.
% To optimize our loss function in Eq.~\eqref{eq:total_loss}, we use stochastic gradient descent (SGD) optimizer with momentum of $0.9$ and weight decay set to $10^{-4}$.
% We use cosine annealing as a learning rate scheduler without warm up.
% We implement in PyTorch and train on a single NVIDIA A100 with 40GB GPU memory.
% In preprocessing, we mostly follow the sequence of \cite{lin2022ocsampler}. To train the model, we randomly scales all frames and randomly crop to a resolution of $224\times224$ with random flipping. The resolution of video frames was further reduced to $128\times128$ for input to $S$. During inference, we continued to use $128\times128$ resolution frames to feed $S$ and averaged the predictions of the center-cropped frames, which were of size $224\times224$. In the absence of specific instructions, we conducted an experiment with $T$=10 and $N$=6. We use MobileNetv2TSM as a feature extractor of the sampler $S$. For the classifier $f_c$, we use ResNet50 \cite{he2016resnet} and TimeSformer \cite{bertasius2021timesformer}. To optimize the loss function, we use stochastic gradient descent (SGD) optimizer. Our model is implemented in PyTorch and was trained on a NVIDIA A100 40GB.

\vspace{0.1cm}
\noindent\textbf{Evaluation Metrics.}
Following the common practice, we measure the mean average precision (mAP), the mean of class average precisions, for ActivityNet, Mini-Sport1M, and COIN datasets.
For Mini-Kinetics, we use top-1 accuracy, which is the ratio of the correctly classified test samples.
%And we use top-1 accuracy, which measures the percentage of test samples that are correctly classified by a model, for Mini-Kinetics and COIN dataset. 
For computational cost, we report GFLOPs for all datasets. % giga-floating-point operation per second (GFLOPs)
%Higher values for mAP and top-1 accuracy are desirable, while lower values indicate better performance for GFLOPs.

% \vspace{0.1cm}
% \noindent\textbf{Baselines.}
% We compare the performance against the \joonseok{current state-of-the-art}, OCSampler~\cite{lin2022ocsampler}, \joonseok{which is built on the same sampling scenario as ours.}
% \joonseok{Since no previous work reports performance with a Transformer-based classifier, we train the OCSampler for TimeSformer on our own, and additionally compare the results against uniform sampling baseline.}
% \joonseok{For ResNet50, we use pretrained weights from \cite{ghodrati2021frameexit} on ActivityNet and Mini-Kinetics, and train from scratch for other datasets.}
%For ActivityNet and Mini-Kinetics datasets, we use the pretrained ResNet50 weights of \cite{ghodrati2021frameexit}.
%\joonseok{We train the classifier from scratch for all other experiments, \textit{i.e.}, ResNet50 on Mini-Sport1M and COIN, and TimeSformer on all datasets.}
%Comparison on the Transformer architecture does note exist in previous methods, so we set uniform sampling as a baseline for both models.
%We choose OCSampler as the comparison target, since it has the same sampling scenario as ours and is the leading approach among the state-of-the-art methods in CNN-based approach.

%and benchmark our proposed method against \red{existing state-of-the-art methods}.
% For other datasets, including Mini-Sport1m, FCVID, and COIN, we train the ResNet50 as a classifier on the specific dataset and use it as a baseline for comparison. 
% For TimeSformer, we train the model for all dataset and use it as a baseline. %For ActivityNet and Mini-Kinetics dataset, we get pretrained weights of ResNet50 from prior works, so we compare our method with existing methods.
%For other datasets, \textit{i.e.}, Mini-Sport1M, and COIN, in ResNet50 and for all datasets in TimeSformer, we train the classifiers $f_c$ on each dataset and use them as baseline models.

%, which has the best performance out of the existing methods.

% \input{tables/resnet_anet_minik_sota}
\input{tables/10to6_performance}
\subsection{Results and Analysis}
\label{sec:exp:results}
\vspace{0.1cm}
% \noindent \textbf{Quantitative Analysis.}

\noindent \textbf{Comparison with Small $N$ and $T$.}
To compare with existing methods under the same conditions,\footnote{Results for OCSampler with ResNet50 in \cref{table:sota_anet_k200} is our reproduction using pre-trained weights and settings provided by the original author. They slightly lag behind on Mini-Kinetics, by 0.7\%.} we first evaluate with the common setting of $T = 10$ and $N = 6$ (except for Mini-Kinetics with ResNet50, where $N = 5$).
%small values of $N$ and $T$.


%\cref{table:sota_anet_k200}--\ref{table:sota_sport_coin} compare our method with baselines on the four datasets using various architectures.
%to demonstrate the generalizability of our approach.
% We report the performance of our model with $T$ set to 10 and $N$ set to 6 for all datasets except Mini-Kinetics, for which $N$ is set to 5.
% We compare with the state-of-the-art backbones listed in \cref{table:sota_anet_k200}--\ref{table:sota_sport_coin} on four datasets, ActivityNet-v1.3, Mini-Kinetics, Mini-Sports1M, and COIN.\footnote{Results for OCSampler with ResNet50 in \cref{table:sota_anet_k200} is our reproduction using pretrained weights and settings provided by the original author. They slightly lag behind on Mini-Kinetics, by 0.7\%.}
% In order to assess the generalizability of our method across diverse architectures, experiments are conducted on a 2D-CNN, ResNet~\cite{he2016resnet}, 3D CNN backbone, SlowOnly-50~\cite{feichtenhofer2019slowfast} and X3D-S~\cite{feichtenhofer2020x3d}, and transfomer, Timesformer~\cite{bertasius2021timesformer}.
% 
%From the result, 

As seen in \cref{table:sota_anet_k200}--\ref{table:sota_sport_coin}, our approach consistently outperforms previous methods across all four datasets and backbone architectures, highlighting the effectiveness of learning $\pi_s$ even when the search space is not very large.
%\junho{These results suggest that learning $\pi_o$ is challenging even when the search space is not very large, }
% we observe that our SOSampler consistently outperforms most baselines across all four datasets and architectures, with relatively lower GFLOPs than most competing models.
Nevertheless, comparing \cref{table:sota_anet_k200} to \cref{tab:oracle_conf_sampler_result}, we observe that SOSampler still does not fully emulate $\pi_s$, possibly due to the loss when it transfers the label information.
A future work may further address this issue to fill the gap.
% \input{tables/resnet_minis_fcvid_coin_sota}

% \vspace{0.1cm}
% \noindent\textbf{Comparison with Transformer Classifiers.}
% We report the performance of our approach with transformer architecture in listed in \cref{table:sota_anet_k200}--\ref{table:sota_sport_coin} on four datasets, ActivityNet-v1.3, Mini-Kinetics, Mini-Sports1M, and COIN.

% Overall, our approach, KDSampler, outperforms both baselines on most datasets for 6 sampled frames per video, achieving mAP of 88.65\% on ActivityNet-v1.3, a top-1 accuracy of 81.62\% on COIN, and an mAP of 50.04\% on Mini-Sports1M.
% It also achieves a top-1 accuracy of 80.52\% on Mini-Kinetics, which is comparable to the results of baselines.

% These results suggest that it is adaptable to the Transformer architecture.
% Surprisingly, however, OCSampler shows worse performance even than the uniform sampling baseline except on Mini-Kinetics, while spending more computational cost.
% Although we do not figure the exact reason, we cautiously assume that the instability of the RL method may have been a problem in the process of switching to a backbone of a completely different structure.
% This result indicates that OCSampler does not translate properly into the Transformer architecture.
% We further evaluate our KDSampler for sampling 3--5 frames per video.
% Although the performance drops as expected, our approach still outperforms uniform sampling baseline using lower GFLOPs.
%KDSampler achieves an mAP of 87.20\% on ActivityNet-v1.3 and a top-1 accuracy of 79.15\% on COIN with 4 frames per video. 

% \vspace{0.1cm}

% \vspace{0.1cm}
%This provides a better understanding of how our sampler is able to effectively sample frames based on their importance scores to improve the efficiency and accuracy of action recognition.
% Results of $S_o$ and $S_c$ for ActivityNet and Mini-Kinetics are shown in Tab.~\ref{tab:oracle_conf_sampler_result}. We report on ResNet50 and TimeSformer model.  

% As we mentioned in Sec.~\ref{sec:method:problem}, we find that sampling policy of $S_c$ approximates $S_o$ both in CNN and Transformer architecture. As shown in Tab.~\ref{tab:oracle_conf_sampler_result}, $S_c$ 
% \input{tables/resnet_minis_fcvid_coin_sota}


\input{figures/large_tn_table_graph}
% \input{tables/tn_ablation_anet_minis}
% \input{tables/tn_ablation_minik_coin}
% \input{figures/anet_uni_oc_kd_tn_comparison}
\vspace{0.1cm}
\noindent\textbf{Comparison with Large $N$ and $T$.}
We conduct experiments on large $N$ and $T$ to verify the effect of reduced search space by our proposed policy $\pi_s$, comparing with OCSampler~\cite{lin2022ocsampler} and uniform sampling as baselines.
Note that OCSampler and SOSampler have exactly the same architecture -- the only difference lies in the learning objective.
We evaluate on the ActivityNet-v1.3 and Mini-Sports1M datasets, which consist of sufficiently long videos\footnote{Results for short videos are discussed in~\cref{appendix:large_nt_short}.}, to ensure the frame independence even for a large $T$.

As shown in \cref{tab:large_tn}, our approach consistently achieves competitive performance regardless of the backbone architectures and with various values of $N$ and $T$.
%achieves good performance even with changes in backbone architectures and increases in $N$ and $T$.
With the OCSampler, on the other hand, the performance improvement is inconsistent and it sometimes underperforms even than the uniform sampling.
%significantly underperforms as $N$ and $T$ increase, the performance gap widens compared to our approach.}
This is illustrated in \cref{fig:anet_tn_graph} as well; the performance of OCSampler lags behind the uniform sampling from $N = 16, T = 60$ and beyond, indicating that directly searching the $O(T^N)$ space is not scalable for large $N$ and $T$.
Our semi-optimal policy does not suffer from this, recalling that our approach adopts the same architecture as OCSampler.
%Particularly, as seen in \cref{fig:anet_tn_graph}, OCSampler's performance degrades compared to uniform sampling from the point of 16/60, indicating a diminishing effectiveness as a sampler.
Additionally, we observe that OCSampler does not perform well with the TimeSformer backbone.
We also attribute this to the more complex search space of transformer-based classifiers compared to CNN-based ones.
Based on the results, we conclude that our approach to reduce the complexity of search space is indeed effective for large $N$ and $T$, which has been challenging for existing methods.
% As seen in \cref{tab:large_tn}, OCSampler demonstrates poorer performance even compared to uniform sampling as $N$ and $T$ increase, indicating that it does not effectively search the vast space.
% Conversely, our approach continues to perform nicely even for the increased $N$ and $T$.
% could effectively reduce the spatial complexity and the difficulty of optimization .
% This confirms that the reduced complexity of the search space indeed helps, allowing effective exploration even when $N$ gets high, in line with our hypothesis.

% \input{figures/qualitative_analysis}

\vspace{0.1cm}
\noindent\textbf{Qualitative Analysis.}
% To better demonstrate how our trained sampler $S_\text{KD}$ succeeds in effective sampling, we qualitatively demonstrate the sampled frames from a few videos in \cref{fig:qualitative_analysis}.
% Same as in the quantitative analysis, the sampler selects 6 frames out of 10 candidate frames.
% %As we previously described, ten video candidates are downsampled and fed as input to $S_\text{KD}$, and the sampler predicts the importance score and extracts the six frames with highest scores.
% In the videos of ``Rock Climbing'' and ``Canoeing'', we see that only frames related to the corresponding action label are selected, discarding irrelevant frames.
% For ``Sailing'' and ``Painting'' videos, our sampler captures all the relevant frames to the action label, but has to sample an irrelevant frame, \emph{i.e.}, putting on life vests for ``Sailing'' and a person explaining for ``Painting'', as it is required to sample 6 frames in total.
% \red{For "Sailing" and "Painting" videos, high-levels related to the action label are selected first, and although they do not seem directly related, they can be seen that they selectively chose the ones that are related.}
In \cref{sec:success_case}--\ref{sec:failure_case}, we illustrate success and failure cases of our SOSampler, comparing with sampling policies of $\pi_o$ and $\pi_s$.
% Qualitative analysis demonstrates that our SOSampler learns to select frames effectively based on importance scores that are directly correlated with predicting the video classification label, as we intend.


%\vspace{-2mm}
\subsection{Ablation Study}
\label{sec:exp:ablation}

% \input{tables/ablation}
\noindent\textbf{Loss function.}
\cref{tab:loss_ablation} reports the result of an ablation study on the loss functions, conducted on ActivityNet-v1.3.
`MSE' and `Ranking' indicate the two choices for $\mathcal{L}_\text{SO}$ presented in \cref{sec:sosampler}, while `Label' and `Max' indicate how we obtain the importance score of each frame $c(\bm{v}_t)$ from the confidence distribution $f_c(\bm{v}_t)$ over all classes.

% while `Label' and `Max' indicate how we aggregate the frame-level scores $f_c(\bm{v}_t)$ to the video-level score $c(\bm{v}_t)$ in Eq.~\eqref{eq:conf-based}.

As we mentioned earlier, the ranking loss in Eq.~\eqref{eq:ranking} outperforms the MSE loss for $\mathcal{L}_\text{SO}$.
We also observe that the max-aggregation leads to stronger performance than the label confidence, probably because it learns consistent scores across features.
The label guidance loss $\mathcal{L}_\text{LG}$ turns out to slightly improve the overall performance.
%In \cref{eq:conf-based}, `Label' and `Max' represent whether the function $c(\cdot)$ should use the label's confidence or the maximum confidence.
%Initially, we trained using only MSE loss for $\mathcal{L}_\text{SO}$, but the performance was unsatisfactory. To incorporate label information, we add label guidance loss $\mathcal{L}_\text{LG}$, which slightly improved performance. 
%However, as it still didn't yield adequate performance, we introduced ranking loss as $\mathcal{L}_\text{SO}$ to enable the sampler to learn the order of importance rather than focusing on the exact score. Additionally, 
%To enable the sampler to learn consistent scores across features, we use the max confidence, resulting in improved performance.
% Our initial approach was to use MSE loss, $\mathcal{L}_\text{MSE}$, but the performance was poor even with auxiliary cross-entropy loss. Instead, we use ranking loss, which penalizes the model if it fails to correctly order a pair of two frames according to importance score, as the knowledge distillation loss, $\mathcal{L}_\text{KD}$. As expected, using $\mathcal{L}_\text{KD}$ leads to higher performance. Auxiliary cross-entropy loss, $\mathcal{L}_\text{CE}$ further improves the model for both of the loss functions. Therefore, we adopt a hybrid loss consisting of ranking loss and cross-entropy loss as a default.

% \input{tables/T_ablation}
\input{tables/ablation_study}
\vspace{0.1cm}
\noindent\textbf{Exploration on $N$ and $T$.}
We fix $N = 6$ and $T = 10$ in \cref{table:sota_anet_k200}--\ref{table:sota_sport_coin} mainly for the purpose of comparison with previous models.
We further explore various combinations of $N \in \{2, 4, 6, 8\}$ and $T \in \{6, 10, 16, 24\}$ to better understand our method.
%However, to provide a better understanding of our approach, we measure the performance with more combinations of $T$ and $N$.
%Specifically, we explore $N = \{2, 4, 6, 8\}$ when $T$ is fixed to 10, and $T = \{6, 10, 16, 24\}$ while $N$ is fixed to 6.
As seen in \cref{tab:t_ablation}, performance consistently improves with a larger $N$, but the gain diminishes beyond $N \ge 6$.
Also in the case of $N=6$, we observe consistently improved performance with larger $T$.
% The increase in $T$ is primarily attributed to the computational load of the lightweight sampler $S_\text{KD}$, resulting in just a slight increase of GFLOPs compared to the increase observed when $N$ increases.





==> arXiv-2409.05260v4/sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:summary}

% In this paper, we introduce a novel perspective of reducing the search space in frame sampling, proposing a Semi-optimal policy that simplifies the search space. And we also propose KDSampler, lightweight network distilled to emulate Semi-optimal policy.

% We experimentally verify that the proposed Semi-optimal policy can approximate the optimal sampling policy in several datasets and architecture. KDSampler exhibits better performance in several datasets and structures. Furthermore, unlike previous methods that struggle under the extreme conditions of large $N$ and $T$, our approach continues to demonstrate robustness. These results support our assertion that reducing spatial complexity indeed lowers the difficulty of optimization.

% Our experimental results suggest that there is still substantial scope for improvement in the sampler, indicating potential for further exploration in future work.

In this paper, we address the scalability challenge of the frame sampling task, proposing our novel novel semi-optimal policy $\pi_s$ to dramatically reduce the search space itself from $O(T^N)$ to $O(T)$, supported by empirical evidence of frame independence.
%Existing methods mainly focused on efficiently exploring the wide search space through reinforcement learning. However, we proposed a novel approach by dramatically reducing the search space itself with the semi-optimal policy $\pi_s$.
Through extensive experiments, we demonstrate that $\pi_s$ effectively approximates the optimal policy.
Furthermore, across all datasets and architectures, the sampler which learns $\pi_s$ instead of $\pi_o$ outperforms existing methods both for small and large $N$ and $T$.
These results suggest that our new approach, which changes the search space itself rather than the exploration method, is more effective than previous approaches.
However, the frame independence assumption we propose does not hold in all scenarios, and there remains potential for further performance improvements in the sampler learning our proposed $\pi_s$. Addressing these limitations will be an important direction for future work.
% However, we still observe room for further improvement even with our $\pi_s$, which we leave as a future work.
%\junho{However, our sampler has not yet fully learned $\pi_s$, indicating room for improvement in the training method in future work.}
% 다만 우리의 방법은 적당한 FPS가 유지된 상태에서 가정이 성립한다.

==> arXiv-2409.05260v4/tables/10to6_performance.tex <==
\begin{table}
    \centering
    \begin{minipage}{0.49\textwidth}{
            % \begin{footnotesize}
            % \vspace{-3mm}
            \centering
            \renewcommand{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{
            \begin{tabular}{l|c|@{\hspace{0.3cm}}cccccc}
            \toprule
            \multirow{2}{*}{Methods} & Back- & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} \\
            & bones & mAP & GFLOPs & Top-1 &  GFLOPs \\
            \midrule
            %AdaFrame \cite{wu2019adaframe} & ResNet & 71.5\% & 79.0 & -- & -- \\
            %ListenToLook \cite{gao2020listen} & ResNet & 72.3\%  & 81.4 & -- & -- \\
            LiteEval \cite{wu2019liteeval}& & 72.7\% & 95.1 & 61.0\% & 99.0  \\ 
            SCSampler \cite{korbar2019scsampler}& & 72.9\%  & 42.0 & 70.8\% & 41.9 \\
            AR-Net \cite{meng2020arnet}& & 73.8\% & 33.5 & 71.7\% & 32.0 \\
            videoIQ \cite{sun2021videoiq}& Res- & 74.8\% & 28.1 & 72.3\% & 20.4 \\
            AdaFocus \cite{wang2022adafocus}& Net50 & 75.0\% & 26.6 & 72.9\% & 38.6 \\
            FrameExit \cite{ghodrati2021frameexit}& & 76.1\% & 26.1 & 72.8\% & 19.7 \\
            % \rowcolor{lavendergray}\textit{Samples from 10 to N} & & & &  \\
            OCSampler \cite{lin2022ocsampler}& & 77.2\% & 25.8 & 73.0\% & {21.6} \\
                                              % & 76.9\% (5) & 21.7 & 72.25\% (4) & 17.5 \\
            \textbf{SOSampler} && {\textbf{77.7\%}}& 25.8 &  {\textbf{73.5\%}}& {21.6} \\
                             % & \junho{77.3\%} (5) & 21.7 &  \junho{72.49\%} (4) & 17.5 \\
            \midrule
            % Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & 84.0\% & 701 & 79.2\% & 738 \\
            % OCSampler~\cite{lin2022ocsampler} &  & 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
            Ada2D \cite{li2021ada2d} & 
            Slow &
            %\multirow{3}{*}{SlowOnly-50} & 
            84.0\% & 701 & 79.2\% & 738 \\
            OCSampler~\cite{lin2022ocsampler} & Only & 87.3\% & 68.2 & 82.6\% & 27.3 \\
            \textbf{SOSampler} & 50 & \textbf{88.0\%} & 64.0 & \textbf{83.0\%} & 27.3 \\
            %\textbf{OCSampler} & SlowOnly-101 & \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
            % todo: k200 pretrained can be improved
            \midrule
            FrameExit \cite{ghodrati2021frameexit} & \multirow{3}{*}{X3D-S} & 86.0\% & 9.8 & -- & -- \\
            OCSampler~\cite{lin2022ocsampler} &  & 86.6\% & 7.9 & -- & -- \\
            \textbf{SOSampler} &  & {\textbf{87.2\%}} & {7.6} & -- & -- \\
            \midrule
            % Uniform  & \multirow{3}{*}{TimeSformer} & 87.1\% & \bf{75.7} & 79.6\% & \bf{75.7} \\
            OCSampler~\cite{lin2022ocsampler} & TimeS- & 83.2\% & {76.8} & 80.7\% & {76.8} \\
            \textbf{SOSampler} & former & \textbf{88.7\%} & 76.8 & 80.7\% & {76.8} \\
            \bottomrule
            % \rowcolor{gray}\textit{Kinetics} & & & & &\\
            % Ada2D \cite{li2021ada2d} & SlowOnly-50 & 84.0\% & 701 & 79.2\% & 738 \\
            % ListenToLook \cite{gao2020listentolook} & R(2+1)D-152 & 89.9\% & 2640 & -- & -- \\
            % MARL \cite{wu2019marl} & SEResNeXt-152 & 90.0\% & 7540 & -- & -- \\
            % OCSampler \cite{lin2022ocsampler} & SlowOnly-50 & 87.3\% & \textbf{68.2} & \textbf{82.6\%} & \textbf{27.3} \\
            % %\textbf{OCSampler} & SlowOnly-101 & \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
            % OCSampler \cite{lin2022ocsampler} & SlowOnly-101 & \textbf{90.1\%} & 593 & - & - \\
            
            % % todo: k200 pretrained can be improved
            % \hline
            % \rowcolor{gray}\textit{Kinetics} & & & & &\\
            % FrameExit \cite{ghodrati2021frameexit} & X3D-S & 86.0\% & 9.8 & -- & -- \\
            % OCSampler \cite{lin2022ocsampler} & X3D-S & \textbf{86.6\%} & \textbf{7.9} & -- & -- \\
            \end{tabular}
            }
            \vspace{0.2cm}
            \captionof{table}{\textbf{Comparison on ActivityNet-v1.3 and Mini-Kinetics for small $N$ and $T$.} The best performing model is 
            \textbf{bold-faced}.}
            \label{table:sota_anet_k200}
        }
    \end{minipage}\hfill
    \begin{minipage}{0.49\textwidth}{
        % \vspace{-2mm}
        % \resizebox{1.0\linewidth}{!}{
        \renewcommand{\tabcolsep}{3pt}
        \resizebox{\linewidth}{!}{
        \centering
        \begin{tabular}{l|c|@{\hspace{0.1cm}}cccc}
            \toprule
            \multirow{2}{*}{Methods} & Back- & \multicolumn{2}{c}{Mini-Sports1M} &  \multicolumn{2}{c}{COIN} \\
            & bones & mAP & GFLOPs & Top-1 &  GFLOPs \\
            % \midrule
            % ResNet50 &&&& \\
            \midrule        
            LiteEval~\cite{wu2019liteeval}& & 44.7\% & 66.2 & - & - \\
            SCSampler~\cite{korbar2019scsampler} && 44.3\% & 42.0 & 79.8\% & 42.0 \\
            AR-Net~\cite{meng2020arnet} & Res- & 45.0\% & 37.6 & - & - \\
            AdaFuse~\cite{meng2021adafuse} & Net50 &  44.1\% & 60.3 & - & - \\ %
            OCSampler~\cite{lin2022ocsampler} & & 46.7\% & 25.8 & 80.1\% & 25.8 \\
            % \midrule
            \textbf{SOSampler} &&{\textbf{48.3\%}} & 25.8 & {\textbf{80.7\%}} & 25.8 \\
            % \midrule
            % TimeSformer &&&& \\
            \midrule
            % Uniform  & \multirow{3}{*}{TimeSfromer} & 48.90\% & 75.73G &  79.88\% & 75.73G \\
            OCSampler \cite{lin2022ocsampler} & TimeS- & 45.6\% & 76.8 & 81.4\% & 76.8  \\
            \textbf{SOSampler} & former & \textbf{49.1\%} & 76.8 & \textbf{87.7\%} & 76.8 \\
            \bottomrule
            \end{tabular}
        }
        \vspace{0.2cm}
        \captionof{table}{\textbf{Comparison on Mini-Sports1M and COIN Comparison on for small $N$ and $T$}. The best performing model is \textbf{bold-faced}.}
        \label{table:sota_sport_coin}
    }
    \end{minipage}
    %\vspace{-4mm}    
\end{table}

==> arXiv-2409.05260v4/tables/3D_CNN.tex <==
\begin{table}[t]
    \centering
    % \begin{footnotesize}
    \caption{\junho{\textbf{Comparison with other methods on 3D-CNNs and Transfromers.} We perform experimental trials utilizing 3D CNNs with the aim of probing the prospect of our approach's generalizability across architectural variations. The best results are \textbf{bold-faced}.}}
    \vspace{-3mm}
    % \setlength{\tabcolsep}{0.85mm}{
    % \vspace{5pt}
    % \renewcommand\arraystretch{1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones}  & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} \\
    && mAP & GFLOPs & Top-1 &  GFLOPs \\
    \midrule
    Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    OCSampler~\cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
    KDSampler (Ours) & SlowOnly-50 & \ \ \textbf{87.5\%} & \textbf{68.2} & \textbf{82.6\%} & \textbf{2.3} \\
    %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % todo: k200 pretrained can be improved
    \midrule
    FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    OCSampler~\cite{lin2022ocsampler} & X3D-S & \ \ 86.6\% & \textbf{7.9} & \ \ -- & -- \\
    KDSampler (Ours) & X3D-S & \ \ \textbf{-\%} & \textbf{7.9} & \ \ -- & -- \\
    \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \label{tab:speed}
    % \end{footnotesize}
    \vspace{-5mm}
\end{table}


==> arXiv-2409.05260v4/tables/T_ablation.tex <==
\begin{table}
    %\label{table:decision_space}
    \centering
    \resizebox{0.7\linewidth}{!}{
        \begin{tabular}{c|cccc|cccc}
        \toprule
        $T$ & \multicolumn{4}{c|}{$10$} & $6$ & $10$ & $16$ & $24$\\
        \midrule
        $N$ & $2$ & $4$ & $6$ & $8$ & \multicolumn{4}{c}{$6$}\\
        \midrule
        mAP & 71.1\% & 76.2\% & 77.7\% & \bf{77.9\%}  & 75.3\% & 77.7\% & 78.2\% & \bf{78.4\%} \\ 
        GFLOPs & \bf{9.3} & 17.6 & 25.8 & 34.1   & \bf{24.7} & 25.8 & 26.4 & 27.2 \\
        \bottomrule
        \end{tabular}
    }
    \vspace{0.2cm}
    \caption{\textbf{Ablation study on $T$ and $N$}. % $T = 6$ is same as uniform sampling.
    }
    \label{tab:t_ablation}
    \vspace{-0.3cm}
\end{table}


==> arXiv-2409.05260v4/tables/ablation.tex <==
% \begin{table}[h]
% \centering
% \small
% \caption{\textbf{Ablation study on different losses on ActivityNet.} The best-performing combination is \textbf{bold-faced}.
% %of $\mathcal{L}_\text{KD}$ and $\mathcal{L}_\text{CL}$ shows the best performance.
% }
% %\vspace{-3mm}
% \begin{tabular}{ccc|c}
%     \toprule
%     $\mathcal{L}_\text{MSE}$ & $\mathcal{L}_\text{KD}$ & $\mathcal{L}_\text{CL}$  & mAP (\%)\\
%     \midrule
%     \checkmark& &  & 87.38 \\
%     % \hline
%     \checkmark&  & \checkmark &87.51 \\
%     % \hline
%     & \checkmark & & 88.21 \\
%     % \hline
%     & \checkmark & \checkmark & \textbf{88.65} \\
%     \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:loss_ablation}
% \end{table}

\begin{table}
    \centering
    \footnotesize
    % \vspace{-3mm}
    \begin{tabular}{cccc|c|c}
        \toprule
        % $\mathcal{L}_{MSE}$ & $\mathcal{L}_{KD}$ & $\mathcal{L}_{CL}$  & mAP (\%)\\
        \multicolumn{4}{c|}{$\bm{\mathcal{L}_\text{KD}}$}  & \multirow{2}{*}{\bm{$\mathcal{L}_\text{CE}$}}  & \multirow{2}{*}{mAP (\%)}\\
        % MSE & Ranking Loss & $\mathcal{L}_{CL}$  & mAP (\%)\\
        % \midrule
        MSE         & Ranking   & Label     & Max           &           & \\
        \midrule
        \checkmark &             &  \checkmark   &           &              &   87.38 \\
        \checkmark &             &  \checkmark   &           & \checkmark   & 87.51 \\
                   & \checkmark  & \checkmark    &           &              & 88.21 \\
                   & \checkmark  &  \checkmark   &           &  \checkmark  & 88.40 \\
                  &\checkmark &                  &  \checkmark    &  \checkmark &\textbf{88.65} \\
        % \hline
        \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \caption{\textbf{Ablation study on different losses on ActivityNet.}}
    \label{tab:loss_ablation}
\end{table}

==> arXiv-2409.05260v4/tables/ablation_study.tex <==
\begin{table}
    \centering
    \begin{minipage}{0.38\textwidth}
        \centering
        \renewcommand{\tabcolsep}{4pt}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{cccc|c|c}
                \toprule
                \multicolumn{4}{c|}{${\mathcal{L}_{\text{SO}}}$} & \multirow{2}{*}{${\mathcal{L}_{\text{LG}}}$} & \multirow{2}{*}{mAP (\%)} \\
                MSE & Ranking & Label & Max & & \\
                \midrule
                \checkmark & & \checkmark & & & 87.38 \\
                \checkmark & & \checkmark & & \checkmark & 87.51 \\
                & \checkmark & \checkmark & & & 88.21 \\
                & \checkmark & \checkmark & & \checkmark & 88.40 \\
                & \checkmark & & \checkmark & \checkmark & \textbf{88.65} \\
                \bottomrule
            \end{tabular}
        }
        \vspace{0.2cm}
        \captionof{table}{\textbf{Ablation study on losses.}}
        \label{tab:loss_ablation}
    \end{minipage}\hfill
    \begin{minipage}{0.58\textwidth}
        \renewcommand{\tabcolsep}{3pt}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{c|cccc|cccc}
                \toprule
                $T$ & \multicolumn{4}{c|}{$10$} & $6$ & $10$ & $16$ & $24$\\
                \midrule
                $N$ & $2$ & $4$ & $6$ & $8$ & \multicolumn{4}{c}{$6$}\\
                \midrule
                mAP & 71.1\% & 76.2\% & 77.7\% & \bf{77.9\%}  & 75.3\% & 77.7\% & 78.2\% & \bf{78.4\%} \\ 
                GFLOPs & \bf{9.3} & 17.6 & 25.8 & 34.1   & \bf{24.7} & 25.8 & 26.4 & 27.2 \\
                \bottomrule
            \end{tabular}
        }
        \vspace{0.2cm}
        \captionof{table}{\textbf{Ablation study on $T$ and $N$.}}
        \label{tab:t_ablation}
    \end{minipage}
\end{table}


% \begin{table}
%     \centering
%     \begin{minipage}{0.38\textwidth}{
%             % \begin{footnotesize}
%             % \vspace{-3mm}
%             \centering
%             \renewcommand{\tabcolsep}{4pt}
%             \resizebox{\linewidth}{!}{
%                 \begin{tabular}{cccc|c|c}
%                     \toprule
%                     % $\mathcal{L}_{MSE}$ & $\mathcal{L}_{KD}$ & $\mathcal{L}_{CL}$  & mAP (\%)\\
%                     \multicolumn{4}{c|}{$\bm{\mathcal{L}_\text{SO}}$}  & \multirow{2}{*}{\bm{$\mathcal{L}_\text{LG}$}}  & \multirow{2}{*}{mAP (\%)}\\
%                     % MSE & Ranking Loss & $\mathcal{L}_{CL}$  & mAP (\%)\\
%                     % \midrule
%                     MSE         & Ranking   & Label     & Max           &           & \\
%                     \midrule
%                     \checkmark &             &  \checkmark   &           &              &   87.38 \\
%                     \checkmark &             &  \checkmark   &           & \checkmark   & 87.51 \\
%                                & \checkmark  & \checkmark    &           &              & 88.21 \\
%                                & \checkmark  &  \checkmark   &           &  \checkmark  & 88.40 \\
%                               &\checkmark &                  &  \checkmark    &  \checkmark &\textbf{88.65} \\
%                     % \hline
%                     \bottomrule
%                 \end{tabular}
%             }
%             \vspace{0.2cm}
%             \captionof{table}{\textbf{Ablation study on  losses.}}
%             \label{tab:loss_ablation}
%         }
%     \end{minipage}\hfill
%     \begin{minipage}{0.58\textwidth}{
%         % \vspace{-2mm}
%         % \resizebox{1.0\linewidth}{!}{
%         \renewcommand{\tabcolsep}{3pt}
%         \resizebox{\linewidth}{!}{
%         \centering
%         \begin{tabular}{c|cccc|cccc}
%         \toprule
%         $T$ & \multicolumn{4}{c|}{$10$} & $6$ & $10$ & $16$ & $24$\\
%         \midrule
%         $N$ & $2$ & $4$ & $6$ & $8$ & \multicolumn{4}{c}{$6$}\\
%         \midrule
%         mAP & 71.1\% & 76.2\% & 77.7\% & \bf{77.9\%}  & 75.3\% & 77.7\% & 78.2\% & \bf{78.4\%} \\ 
%         GFLOPs & \bf{9.3} & 17.6 & 25.8 & 34.1   & \bf{24.7} & 25.8 & 26.4 & 27.2 \\
%         \bottomrule
%         \end{tabular}
%         }
%         \vspace{0.2cm}
%         \captionof{table}{\textbf{Ablation study on $T$ and $N$}. % $T = 6$ is same as uniform sampling.
%         }
%         \label{tab:t_ablation}
%     }
%     \end{minipage}
%     %\vspace{-4mm}    
% \end{table}

==> arXiv-2409.05260v4/tables/anet_x3d.tex <==
\begin{table}[t]
    \caption{\textbf{X3D-S Comparison on ActivityNet}.} % $T = 6$ is same as uniform sampling.
    \vspace{-3mm}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{l|cc}
        \toprule
        Method & mAP & GFLOPs\\
        \midrule
        Baseline & 65.1\% & - \\
        OCSampler~\cite{lin2022ocsampler} & 66.3\% & 7.9 \\
        \textbf{KDSampler} & \textbf{68.5\%} & 7.9 \\ 
        \textbf{KDSampler} & 67.1\% & \textbf{7.5} \\ 
        \bottomrule
    \end{tabular}
    }
    \label{table:anet_x3d}
    \vspace{-5mm}
\end{table}


==> arXiv-2409.05260v4/tables/failure_cases.tex <==
\begin{figure*}[h]
    \centering 
    \includegraphics[width=1.0\textwidth]{files/failure_cases_5.drawio.png} 
    \vspace{0.2cm}
    \caption{\textbf{Sampling policy comparison with $\pi_s$, $\pi_o$ for failure cases of SOSampler.}
    }
    \label{fig:fail}
\end{figure*}

==> arXiv-2409.05260v4/tables/large_t_n.tex <==

\begin{table}
    \caption{\textbf{Comparison with large $T$ and $N$}.}
    % \vspace{-3mm}
    \footnotesize
    \centering
        \begin{tabular}{l|cccc}
        \toprule
        \multicolumn{1}{c|}{$T$} & 30 & 60 & 100 & 100 \\
        \multicolumn{1}{c|}{$N$} & 16 & 16 & 16 & 32 \\
        \midrule
        Uniform sampler & 79.2\% & 79.2\% & 79.2\% & 80.2\% \\
        OCSampler~\cite{lin2022ocsampler} & 78.6\% & 78.2\% & 77.9\% & 79.2\% \\
        KDSampler (Ours) & \textbf{80.0\%} & \textbf{80.2\%} & \textbf{80.5\%} & \textbf{81.0\%} \\
        \bottomrule
        \end{tabular}
    \label{tab:ablation_t_n_large}
    % \vspace{-2mm}
\end{table}


==> arXiv-2409.05260v4/tables/oracle_conf_indice.tex <==
\begin{table}
    \centering
    \caption{\textbf{Sampling Fidelity}. 
    Note that we report the expected value of the sampling fidelity for random sampling.
    % We report the sampling fidelity, which indicates the similarity of the sampled set to the oracle set, across various values of $N$. Note that we report the expected value of the sampling fidelity for random sampling. All the policies employ the same classifier and frame candidates, with $T$ fixed at 10.
    }
    \label{tab:fidelity}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|c|cccccc}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampler} & \multicolumn{6}{c}{Sampling Fidelity} \\ 
                             &                          & $N=$~1& $N=$~2& $N=$~3& $N=$~4& $N=$~5& $N=$~6    \\ \midrule
    \multirow{3}{*}{ActivityNet} & Random                 & 0.100  & 0.200  & 0.300  & 0.400  & 0.500 & 0.600  \\ 
                             & FrameExit                & 0.102 & 0.193 & 0.293 & 0.393 & 0.496 & 0.593\\ %\cline{2-8} 
                             & $\pi_s$                      & 1.000    & 0.74 & 0.73 & 0.75 & 0.78 & 0.81 \\ \midrule
    \multirow{3}{*}{Mini-Kinetics} & Random                & 0.100  & 0.200  & 0.300  & 0.400  & 0.500  & 0.600 \\
                             & FrameExit                & 0.098& 0.225& 0.320& 0.425& 0.515& 0.625\\ %\cline{2-8} 
                             & $\pi_s$                     & 1.00    & 0.61 & 0.65 & 0.70  & 0.71  & 0.80  \\ 
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.3cm}
\end{table}

% \begin{table}[h]
% \centering
% \caption{Number of Sampled Frames Data}
% \label{tab:sampled_frames}
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%     \hline
%     \multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampler} & \multicolumn{6}{c|}{Number of sampled frames} \\ \cline{3-8} 
%                              &                          & 1    & 2    & 3    & 4    & 5    & 6    \\ \hline
%     \multirow{3}{*}{ActivityNet} & Random                 & 0.1  & 0.2  & 0.3  & 0.4  & 0.5  & 0.6  \\ \cline{2-8} 
%                              & FrameExit                & 0.099& 0.225& 0.32 & 0.425& 0.515& 0.625\\ \cmidrule{3-8} 
%                              & S\_c                      & 1    & 0.74 & 0.73 & 0.75 & 0.78 & 0.81 \\ \hline
%     \multirow{3}{*}{Mini-Kinetics} & Random                & 0.1  & 0.2  & 0.3  & 0.4  & 0.5  & 0.6  \\ \cline{2-8} 
%                              & FrameExit                & 0.101& 0.193& 0.293& 0.393& 0.496& 0.593\\ \cmidrule{3-8} 
%                              & S\_c                      & 1    & 0.61 & 0.65 & 0.7  & 0.7  & 0.8  \\ \hline
%     \end{tabular}
% \end{table}

==> arXiv-2409.05260v4/tables/oracle_conf_perform.tex <==
\begin{table}
    \begin{center}
    \caption{\textbf{Performance of $\pi_o$ and $\pi_s$ on ActivityNet-v1.3 and Mini-Kinetics}. \junho{Relative improvement from $\pi_u$ is provided on the right side.}
    % We report the performance of the classifier, depending on the different sampling policies of the uniform policy $\pi_u$, oracle policy $\pi_o$, semi-optimal policy $\pi_s$, and input all candidate frames. (Relative improvement from $\pi_u$ is provided as well.) Given $T=10$ candidate frames, each policy selects $N=6$ frames using their sampling policy. Note that classifiers are fixed and only the sampling policy is varied. The results indicate that $\pi_s$ can effectively approximate $\pi_o$ for all benchmarks.
    }
    \vspace{-0.2cm}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|c|cr|cr}
        \toprule
        $f_c$ & Policy & \multicolumn{2}{c|}{ActivityNet (mAP)} & \multicolumn{2}{c}{Mini-Kinetics (Top-1)} \\
        %\midrule 
        %\multicolumn{3}{c}{\textit{ResNet50}} \\
        \midrule
        \multirow{4}{*}{TimeSformer} & $\pi_u$ & 87.09\% & -- & 79.62\% & --\\
        & $\pi_o$ &  91.59\% & +4.50 & 89.36\% & +9.66\\
        & $\pi_s$ &  89.35\% & +2.26 & 84.77\% & +5.15\\
        & All & 89.00\% & +1.91 & 81.23\% & +1.61\\
        \midrule
        \multirow{4}{*}{ResNet50} & $\pi_u$ & 75.33\% & -- & 72.54\% & -- \\
        & $\pi_o$ &  90.54\% & +15.21 & 83.84\% & +11.30 \\
        & $\pi_s$ &  87.44\% & +12.11 & 80.27\% & +7.73 \\
        & All & 77.89\% & +2.56 & 73.64\% & +1.10 \\
        %\midrule 
        %\multicolumn{3}{c}{\textit{TimeSformer}} \\
        \bottomrule
        \end{tabular}
    }
    \vspace{-0.6cm}
    \label{tab:oracle_conf_sampler_result}
    \end{center} 
\end{table}

==> arXiv-2409.05260v4/tables/oracle_conf_performance_fidelity.tex <==
\begin{table}
    \centering
    \begin{minipage}{0.47\textwidth}{
        \centering
        \renewcommand{\tabcolsep}{4pt}
        \resizebox{1.0\linewidth}{!}{
            \begin{tabular}{c|c|rr|cr}
            \toprule
            $f_c$ & Policy & \multicolumn{2}{c|}{A-Net (mAP)} & \multicolumn{2}{c}{M-Kin. (Top-1)} \\
            %\midrule 
            %\multicolumn{3}{c}{\textit{ResNet50}} \\
            \midrule
            \multirow{4}{*}{TimeSformer} & $\pi_u$ & 87.0\% & -- & 79.6\% & --\\
            & $\pi_o$ &  91.5\% & +4.5 & 89.3\% & +9.7\\
            & $\pi_s$ &  89.4\% & +2.4 & 84.8\% & +5.2\\
            & All & 89.0\% & +2.0 & 81.2\% & +1.6\\
            \midrule
            \multirow{4}{*}{ResNet50} & $\pi_u$ & 75.3\% & -- & 72.5\% & -- \\
            & $\pi_o$ &  90.5\% & +15.2 & 83.8\% & +11.3 \\
            & $\pi_s$ &  87.4\% & +12.1 & 80.3\% & +7.8 \\
            & All & 77.8\% & +2.5 & 73.6\% & +1.1 \\
            %\midrule 
            %\multicolumn{3}{c}{\textit{TimeSformer}} \\
            \bottomrule
            \end{tabular}
        }
        \vspace{0.01cm}
        \caption{\textbf{Performance of $\pi_o$ and $\pi_s$ on ActivityNet and Mini-Kinetics}. Relative improvement from $\pi_u$ is provided on the right.}
        \label{tab:oracle_conf_sampler_result}
    }
    \end{minipage}\hfill
    \begin{minipage}{0.51\textwidth}{
        \centering
        \renewcommand{\tabcolsep}{3pt}
        \resizebox{1.0\linewidth}{!}{
            \begin{tabular}{c|c|cccccc}
                \toprule
                \multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampler} & \multicolumn{6}{c}{Sampling Fidelity (\%)} \\ 
                                         &                          & $N=$~1& $N=$~2& $N=$~3& $N=$~4& $N=$~5& $N=$~6    \\ \midrule
                \multirow{3}{*}{A-Net} & Random                 & 10.0  & 20.0  & 30.0  & 40.0  & 50.0 & 60.0  \\ 
                                         & FrameExit                & 10.2 & 19.3 & 29.3 & 39.3 & 49.6 & 59.3 \\ %\cline{2-8} 
                                         & $\pi_s$                      & 100.0    & 74.6 & 73.2 & 75.1 & 78.5 & 81.0 \\ \midrule
                \multirow{3}{*}{M-Kin.} & Random                & 10.0  & 20.0  & 30.0  & 40.0  & 50.0 & 60.0 \\
                                         & FrameExit                & 9.8& 22.5& 32.0 & 42.5 & 51.5 & 62.5 \\ %\cline{2-8} 
                                         & $\pi_s$                     & 100.0    & 61.5 & 65.2 & 70.6  & 71.8  & 80.5  \\ 
                \bottomrule
            \end{tabular}
        }
        \vspace{0.1cm}
        \caption{\textbf{Sampling Fidelity}. 
        Note that we report the expected value of the sampling fidelity for random sampling.
        }
        \label{tab:fidelity}
    }
    \end{minipage}
    %\vspace{-0.4cm}
\end{table}

==> arXiv-2409.05260v4/tables/resnet_anet_minik_sota.tex <==
% \begin{table}[t]
%     \centering
%     % \begin{footnotesize}
%     \caption{\textbf{Comparison on ActivityNet-v1.3 and Mini-Kinetics.} The best performing model is \textbf{bold-faced}.}
%     \label{table:sota_anet_k200}
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{l|c|cccccccccc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} &  \multicolumn{2}{c}{Mini-Sports1M} &  \multicolumn{2}{c}{COIN} \\
%     & & mAP & GFLOPs & Top-1 &  GFLOPs & mAP & GFLOPs & mAP & GFLOPs\\
%     \midrule
%     %AdaFrame \cite{wu2019adaframe} & ResNet & \ \ 71.5\% & 79.0 & \ \ -- & -- \\
%     %ListenToLook \cite{gao2020listen} & ResNet & \ \ 72.3\%  & 81.4 & -- & -- \\
%     LiteEval \cite{wu2019liteeval}& \multirow{8}{*}{ResNet} & \ \ 72.7\% & 95.1 & \ \ 61.0\% & 99.0 &  44.7\%  & 66.2  & -- & --\\ 
%     SCSampler \cite{korbar2019scsampler}& & \ \ 72.9\%  & 42.0 & \ \ 70.8\% & 41.9 & 44.3\% & 42.0 & 73.89\% & 42.0 \\
%     AR-Net \cite{meng2020arnet}& & \ \ 73.8\% & 33.5 & \ \ 71.7\% & 32.0 & 45.0\% & 37.6 & -- & -- \\
%     AdaFuse \cite{meng2021adafuse} & & -- & -- & -- & -- &  44.1\% & 60.3 & -- & -- \\
%     videoIQ \cite{sun2021videoiq}& & \ \ 74.8\% & 28.1 & \ \ 72.3\% & 20.4 & -- & -- & -- & -- \\
%     AdaFocus \cite{wang2022adafocus}& & \ \ 75.0\% & 26.6 & \ \ 72.9\% & 38.6 & -- & -- & -- & -- \\
%     FrameExit \cite{ghodrati2021frameexit}& & \ \ 76.1\% & 26.1 & \ \ 72.8\% & \bf{19.7} & -- & -- & -- & -- \\
%     % \rowcolor{lavendergray}\textit{Samples from 10 to N} & & & &  \\
%     OCSampler \cite{lin2022ocsampler}& & \ \ 77.2\% & \textbf{25.8} & \ \ 73.0\% & {21.6} & 46.7\% & 25.7 & 74.28\% & 25.8 \\
%                                       % & \ \ 76.9\% (5) & 21.7 & \ \ 72.25\% (4) & 17.5 \\
%     \textbf{KDSampler} && \ \ {\textbf{77.7\%}}& \textbf{25.8} & \ \  {\textbf{73.5\%}}& {21.6} &{\textbf{47.5\%}} & 25.7 & {\textbf{74.89\%}} & 25.8\\
%                      % & \ \ \junho{77.3\%} (5) & 21.7 & \ \  \junho{72.49\%} (4) & 17.5 \\
%     \midrule
%     % Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
%     % OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
%     Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 & \ \ -- & --  & \ \ -- & --\\
%     OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & 68.2 & 82.6\% & 27.3 & \ \ -- & --  & \ \ -- & --\\
%     \textbf{KDSampler} &  & \ \ \textbf{88.0\%} & \textbf{64.0} & \textbf{83.0\%} & 27.3 & \ \ -- & --  & \ \ -- & --\\
%     %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
%     % todo: k200 pretrained can be improved
%     \midrule
%     FrameExit \cite{ghodrati2021frameexit} & \multirow{3}{*}{X3D-S} & \ \ 86.0\% & 9.8 & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     OCSampler~\cite{lin2022ocsampler} &  & \ \ 86.6\% & 7.9 & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     \textbf{KDSampler} &  & \ \ {\textbf{87.2\%}} & {\textbf{7.6}} & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     \midrule
%     % Uniform  & \multirow{3}{*}{TimeSformer} & \ \ 87.1\% & \bf{75.7} & \ \ 79.6\% & \bf{75.7} \\
%     OCSampler~\cite{lin2022ocsampler} & \multirow{2}{*}{TimeSformer} & \ \ 83.2\% & {76.8} & \ \ 80.7\% & {76.8} & 45.69\% & 76.77 & 79.27\% & 76.77\\
%     \textbf{KDSampler} &  & \ \ \textbf{88.1\%} & \textbf{64.16} & \ \ 80.7\% & {76.8} & \textbf{49.05\%} & \textbf{64.16} & \textbf{80.81\%} & \textbf{64.16} \\
%     \bottomrule
%     % \rowcolor{gray}\textit{Kinetics} & & & & &\\
%     % Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
%     % ListenToLook \cite{gao2020listentolook} & R(2+1)D-152 & \ \ 89.9\% & 2640 & -- & -- \\
%     % MARL \cite{wu2019marl} & SEResNeXt-152 & \ \ 90.0\% & 7540 & -- & -- \\
%     % OCSampler \cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & \textbf{82.6\%} & \textbf{27.3} \\
%     % %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
%     % OCSampler \cite{lin2022ocsampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 593 & - & - \\
    
%     % % todo: k200 pretrained can be improved
%     % \hline
%     % \rowcolor{gray}\textit{Kinetics} & & & & &\\
%     % FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
%     % OCSampler \cite{lin2022ocsampler} & X3D-S & \ \ \textbf{86.6\%} & \textbf{7.9} & \ \ -- & -- \\
%     \end{tabular}
%     }
%     % \vspace{-0.6cm}
% \end{table}

\begin{table}[t]
    \centering
    % \begin{footnotesize}
    \caption{\textbf{Comparison on ActivityNet-v1.3 and Mini-Kinetics.} The best performing model is \textbf{bold-faced}.}
    \label{table:sota_anet_k200}
    % \vspace{-3mm}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} \\
    & & mAP & GFLOPs & Top-1 &  GFLOPs \\
    \midrule
    %AdaFrame \cite{wu2019adaframe} & ResNet & \ \ 71.5\% & 79.0 & \ \ -- & -- \\
    %ListenToLook \cite{gao2020listen} & ResNet & \ \ 72.3\%  & 81.4 & -- & -- \\
    LiteEval \cite{wu2019liteeval}& \multirow{8}{*}{ResNet} & \ \ 72.7\% & 95.1 & \ \ 61.0\% & 99.0  \\ 
    SCSampler \cite{korbar2019scsampler}& & \ \ 72.9\%  & 42.0 & \ \ 70.8\% & 41.9 \\
    AR-Net \cite{meng2020arnet}& & \ \ 73.8\% & 33.5 & \ \ 71.7\% & 32.0 \\
    videoIQ \cite{sun2021videoiq}& & \ \ 74.8\% & 28.1 & \ \ 72.3\% & 20.4 \\
    AdaFocus \cite{wang2022adafocus}& & \ \ 75.0\% & 26.6 & \ \ 72.9\% & 38.6 \\
    FrameExit \cite{ghodrati2021frameexit}& & \ \ 76.1\% & 26.1 & \ \ 72.8\% & \bf{19.7} \\
    % \rowcolor{lavendergray}\textit{Samples from 10 to N} & & & &  \\
    OCSampler \cite{lin2022ocsampler}& & \ \ 77.2\% & \textbf{25.8} & \ \ 73.0\% & {21.6} \\
                                      % & \ \ 76.9\% (5) & 21.7 & \ \ 72.25\% (4) & 17.5 \\
    \textbf{KDSampler} && \ \ {\textbf{77.7\%}}& \textbf{25.8} & \ \  {\textbf{73.5\%}}& {21.6} \\
                     % & \ \ \junho{77.3\%} (5) & 21.7 & \ \  \junho{72.49\%} (4) & 17.5 \\
    \midrule
    % Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    % OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
    Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & 68.2 & 82.6\% & 27.3 \\
    \textbf{KDSampler} &  & \ \ \textbf{88.0\%} & \textbf{64.0} & \textbf{83.0\%} & 27.3 \\
    %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % todo: k200 pretrained can be improved
    \midrule
    FrameExit \cite{ghodrati2021frameexit} & \multirow{3}{*}{X3D-S} & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    OCSampler~\cite{lin2022ocsampler} &  & \ \ 86.6\% & 7.9 & \ \ -- & -- \\
    \textbf{KDSampler} &  & \ \ {\textbf{87.2\%}} & {\textbf{7.6}} & \ \ -- & -- \\
    \midrule
    % Uniform  & \multirow{3}{*}{TimeSformer} & \ \ 87.1\% & \bf{75.7} & \ \ 79.6\% & \bf{75.7} \\
    OCSampler~\cite{lin2022ocsampler} & \multirow{2}{*}{TimeSformer} & \ \ 83.2\% & {76.8} & \ \ 80.7\% & {76.8} \\
    \textbf{KDSampler} &  & \ \ \textbf{88.1\%} & \textbf{64.16} & \ \ 80.7\% & {76.8} \\
    \bottomrule
    % \rowcolor{gray}\textit{Kinetics} & & & & &\\
    % Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    % ListenToLook \cite{gao2020listentolook} & R(2+1)D-152 & \ \ 89.9\% & 2640 & -- & -- \\
    % MARL \cite{wu2019marl} & SEResNeXt-152 & \ \ 90.0\% & 7540 & -- & -- \\
    % OCSampler \cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & \textbf{82.6\%} & \textbf{27.3} \\
    % %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % OCSampler \cite{lin2022ocsampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 593 & - & - \\
    
    % % todo: k200 pretrained can be improved
    % \hline
    % \rowcolor{gray}\textit{Kinetics} & & & & &\\
    % FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    % OCSampler \cite{lin2022ocsampler} & X3D-S & \ \ \textbf{86.6\%} & \textbf{7.9} & \ \ -- & -- \\
    \end{tabular}
    }
    % \vspace{-0.6cm}
\end{table}

==> arXiv-2409.05260v4/tables/resnet_minis_fcvid_coin_sota.tex <==
\begin{table}
    \begin{center}
    \caption{\textbf{Comparison with competing models on Mini-Sports1M and COIN}. The best performing model is \textbf{bold-faced}.}
    % \vspace{-2mm}
    \resizebox{0.5\linewidth}{!}{
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|@{\hspace{0.4cm}}cccc}
        \toprule
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{Mini-Sports1M} &  \multicolumn{2}{c}{COIN} \\
        & & mAP & GFLOPs & Top-1 &  GFLOPs \\
        % \midrule
        % ResNet50 &&&& \\
        \midrule        
        LiteEval~\cite{wu2019liteeval}& \multirow{6}{*}{ResNet50} & 44.7\% & 66.2 & - & - \\
        SCSampler~\cite{korbar2019scsampler} && 44.3\% & 42.0 & 73.89\% & 42.0 \\
        AR-Net~\cite{meng2020arnet} && 45.0\% & 37.6 & - & - \\
        AdaFuse~\cite{meng2021adafuse} &&  44.1\% & 60.3 & - & - \\ %
        OCSampler~\cite{lin2022ocsampler} && 46.7\% & 25.7 & 74.28\% & 25.8 \\
        % \midrule
        \textbf{KDSampler} (ours) &&{\textbf{47.5\%}} & 25.7 & {\textbf{74.89\%}} & 25.8 \\
        % \midrule
        % TimeSformer &&&& \\
        \midrule
        % Uniform  & \multirow{3}{*}{TimeSfromer} & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        OCSampler \cite{lin2022ocsampler} & \multirow{2}{*}{TimeSfromer}& 45.69\% & 76.77 & 79.27\% & 76.77  \\
        \textbf{KDSampler} (ours) && \textbf{49.05\%} & \textbf{64.16} & \textbf{80.81\%} & \textbf{64.16} \\
        \bottomrule
        \end{tabular}
    } 
    \vspace{-2mm}
    \label{table:sota_sport_coin}
    \end{center} 
    \vspace{-2mm}
\end{table}

% \begin{table}
%     \begin{center}
%     \caption{\small \textbf{Improvement comparison from baseline on Mini-Sports1M and FCVID}. OCSampler achieves the best mAP while offering significant savings in GFLOPs.}
%     \vspace{-2mm}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccccc}
%         \hline
%         \multirow{2}{*}{Methods} &  \multicolumn{2}{c}{Mini-Sports1M} & \multicolumn{2}{c}{FCVID} & \multicolumn{2}{c}{COIN}  \\
%         &  mAP & GFLOPs  &  mAP & GFLOPs  &  Top-1 & GFLOPs \\
%         \hline 
%         \hline 
%         Baseline (ResNet50) & 39.98\% & 24.7 & --\% & 24.7 & 73.91 & 24.7 \\
%         OCSampler \cite{lin2022ocsampler} & --\% & 25.8 & --\% & 25.8 & 74.28 & 25.8 \\
%         KDSampler  & 40.87\% & 25.8 & --\% & 25.8 & 74.89 & 25.8 \\
%         % LiteEval~\cite{wu2019liteeval} & 44.7\% & 66.2 & 80.0\% & 94.3 \\
%         % SCSampler~\cite{korbar2019scsampler} & 44.3\% & 42.0 & 81.0\% & 42.0 \\
%         % AR-Net~\cite{meng2020ar} & 45.0\% & 37.6 & 81.3\% & 35.1 \\
%         % AdaFuse~\cite{meng2020adafuse} &  44.1\% & 60.3 & 81.6\% & 45.0 \\ %
%         % \hline
%         \hline
%         \end{tabular}
%     } 
%     \vspace{-2mm}
%     \label{table:sota_actv_fcvid}
%     \end{center} 
%     %\vspace{-5mm}
% \end{table}

==> arXiv-2409.05260v4/tables/success_cases.tex <==
\begin{figure*}[h]
    \centering 
    \includegraphics[width=1.0\textwidth]{files/success_cases.drawio.png} 
    \vspace{0.2cm}
    \caption{\textbf{Sampling policy comparison with $\pi_s$, $\pi_o$ for success cases of SOSampler.}
    }
    \label{fig:success}
\end{figure*}

==> arXiv-2409.05260v4/tables/throughput.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    %\vspace{-3mm}
    % \scalebox{1}{
        \begin{tabular}{l|@{\hspace{0.4cm}}cccc}
        \toprule
        \multirow{2}{*}{Methods} & \multirow{2}{*}{mAP} & \multirow{2}{*}{GFLOPs} &  \multicolumn{2}{c}{Throughput}\\
        &&& (Videos/s) \\
        \midrule
        %LiteEval~\cite{wu2019liteeval} & ResNet-50 & 72.7\% & 95.1 & 3.6 \\
        AdaFrame~\cite{wu2019adaframe} & 71.5\% & 79.0 & 6.4 \\
        FrameExit~\cite{ghodrati2021frameexit} & 76.1\% & 26.1 & 19.1 \\
        AR-Net~\cite{meng2020arnet} & 73.8\% & 33.4 & 23.1 \\
        AdaFocus~\cite{wang2022adafocus} & 75.0\% & 26.6 & 44.9 \\
        % OCSampler~\cite{lin2022ocsampler} & 76.9\% & 21.7 & 123.9 \\
        OCSampler~\cite{lin2022ocsampler} & 77.2\% & 25.8 & 107.7 \\
        \textbf{SOSampler} (ours) &\textbf{77.3\%} & \textbf{21.6} & \textbf{123.9} \\
        \bottomrule
        \end{tabular}
        % \begin{tabular}{cccccc}
        % \hline
        % \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multirow{2}{*}{mAP} & \multirow{2}{*}{GFLOPs} &  \multicolumn{2}{c}{Throughput}\\
        % &&&& (Videos/s) \\
        % \hline
        % %LiteEval~\cite{wu2019liteeval} & ResNet-50 & 72.7\% & 95.1 & 3.6 \\
        % AdaFrame~\cite{wu2019adaframe} & MN+R50 & 71.5\% & 79.0 & 6.4 \\
        % FrameExit~\cite{ghodrati2021frameexit} & ResNet-50 & 76.1\% & 26.1 & 19.1 \\
        % AR-Net~\cite{meng2020arnet} & MN+RN & 73.8\% & 33.4 & 23.1 \\
        % AdaFocus~\cite{wang2022adafocus} & MN+RN & 75.0\% & 26.6 & 44.9 \\
        % OCSampler & MN-T+R50 & 77.2\% & 25.8 & 107.7 \\
        % KDSampler & MN-T+R50 & \textbf{77.3\%} & \textbf{21.7} & \textbf{123.9} \\
        % \end{tabular}
    % } 
    \vspace{0.2cm}
    \caption{\textbf{Comparison of computational overhead} in GFLOPs and throughput. (ResNet50 on ActivityNet)}
    \label{tab:throughput}
    %\vspace{-3mm}
\end{table}

==> arXiv-2409.05260v4/tables/timesformer.tex <==
\begin{table*}
    \vspace{-0.2cm}
    \begin{center}
    \caption{
    \textbf{Comparison with TimeSformer Classifiers.} We report performance of our approach compared to uniform sampling and OCSampler \cite{lin2022ocsampler}, which is the SOTA frame sampler in CNN architecture on ActivityNet-v1.3, Mini-Kinetics, Mini-Sports1M, and COIN. Although OCSampler works well with CNNs, it fails to outperform even uniform sampling with Transformer classifiers except on Mini-Kinetics dataset. However, our approach shows great performance on all datasets with the Transformer architecture. 
    % However, our apporoach still do not approach to teacher sampler $S_c$
    }
    \vspace{-0.2cm}
    \begin{footnotesize}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccccc}
        \toprule
        \multirow{2}{*}{Methods (T/N)} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} &  \multicolumn{2}{c}{Mini-Sports1M} & \multicolumn{2}{c}{COIN} \\
        & mAP & GFLOPs & Top-1 & GFLOPs & mAP & GFLOPs & Top-1 & GFLOPs\\
        \midrule
        Uniform (6/-) & 87.09\% & 75.73G & 79.62\% & 75.73G & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        % Uniform (10/-) & 87.09\% & 75.73G & 79.62\% & 75.73G & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        OCSampler (6/10) \cite{lin2022ocsampler} & 83.20\% & 76.77G & \textbf{80.66\%} & 76.77G & 45.69\% & 76.77G &  79.27\% & 76.77G \\
        KDSampler (5/10) & 88.13\% & 64.16G & 79.75\% & 64.16G & 49.05\% & 64.16G & 80.81\% & 64.16G \\
        ~~~~~~~~~~~~~~~~~~~ (6/10) & \textbf{88.65\%} & 76.77G & 80.52\% & 76.77G & \textbf{50.04\%} & 76.77G &  \textbf{81.62\%} & 76.77G\\
        % \midrule
        
        \bottomrule
        \end{tabular}
    %} 
    \vspace{-0.4cm}
    \label{table:timesformer_sota}
    \end{footnotesize}
    \end{center} 
\end{table*}

==> arXiv-2409.05260v4/tables/tn_ablation_anet_minis.tex <==
\begin{table}[htbp]
    \centering
    \label{tab:tn_ablation}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{@{}l|l|l|ccc@{}}
    \toprule
    \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{$N$~/~$T$} \\
    % \cmidrule(l){4-6}
                                 &                           &         & 8~/~30          & 16~/~60         & 32~/~100         \\ 
    \midrule
    \multirow{6}{*}{ActivityNet} & \multirow{4}{*}{ResNet}      & Uniform           & 77.19        & 79.45        & 80.40        \\
                                 % &                              & Random            & 75.68        & 78.97        & 80.12        \\
                                 &                              & OCSampler         & 78.01        & 79.10        & 80.10        \\
                                 &                              & KDSampler         & \textbf{78.65}        & \textbf{80.20}        & \textbf{81.10}        \\ 
    \cmidrule(l){2-6}
                                 & \multirow{4}{*}{TimeSformer}  & Uniform           & 88.51        & 89.90        & 90.30        \\
                                 % &                              & Random            & 87.48        & 89.07        & 90.06        \\
                                 &                              & OCSampler         & 85.06        & 85.38        & 84.53        \\
                                 &                              & KDSampler         & \textbf{89.54}        & \textbf{90.06}        & \textbf{90.45}        \\ 
    \midrule
    \multirow{6}{*}{Mini-Sports1M} & \multirow{4}{*}{ResNet} & Uniform  & 46.95 & 48.89 & 49.18 \\
                                 % &  & Random  & 46.09 & 48.69 & 48.92 \\
                                 &  & OCSampler  & 48.62 & 49.62 & 50.09 \\
                                 &  & KDSampler  & \textbf{50.00} & \textbf{51.10} & \textbf{51.46} \\
    \cmidrule(l){2-6}
                                 & \multirow{4}{*}{TimeSformer} & Uniform  & 53.97 & 55.60 & 56.85 \\
                                 % &  & Random  & 52.94 & 56.55 & 57.79 \\
                                 &  & OCSampler & 48.93 & 49.62 & 50.03 \\
                                 &  & KDSampler & \textbf{55.11} & \textbf{56.85} & \textbf{57.75} \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Experiment on long video datasets for large $T$ and $N$}. The best performing model is \textbf{bold-faced}.}
\end{table}


==> arXiv-2409.05260v4/tables/tn_ablation_minik_coin.tex <==
\begin{table}[t]
    \centering
    \label{tab:tn_ablation}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}l|l|l|ccc@{}}
    \toprule
    \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{$N$~/~$T$} \\
    % \cmidrule(l){4-6}
                                 &                           &                   & 8~/~30          & 16~/~60   & 32~/~100         \\ 
    \midrule
    \multirow{4}{*}{Mini-Kinetics} & \multirow{2}{*}{ResNet} & OCSampler   & 73.52\%  & 74.00\%  & 74.17\%  \\
                                 &                              & SOSampler   & \textbf{73.79\%}  & \textbf{74.46\%}  & \textbf{74.65\%}  \\
    \cmidrule(l){2-6}
                                 & \multirow{2}{*}{TimeSformer} & OCSampler        & 79.13\%  & 78.05\%  & 76.33\%  \\
                                 &                              & SOSampler         & \textbf{79.93\%}  & \textbf{80.44\%}  & \textbf{81.32\%}  \\ 
    \midrule
    \multirow{4}{*}{COIN} & \multirow{2}{*}{ResNet} & OCSampler  & 78.69\% & 79.79\% & 80.06\% \\
                         &  & SOSampler  & \textbf{79.13\%} & \textbf{80.21\%} & \textbf{81.02\%} \\
    \cmidrule(l){2-6}
     & \multirow{2}{*}{TimeSformer} & OCSampler  & 80.88\% & 80.90\% & 81.20\% \\
                                 &  & SOSampler  & \textbf{86.52\%} & \textbf{87.37\%} & \textbf{88.08\%} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{0.2cm}
    \captionof{table}{\textbf{Experiment on short video datasets for large $N$ and $T$}. The best performing model is \textbf{bold-faced}.}
    \label{tab:short_video}
\end{table}
% \begin{table}[htbp]
%     \centering
%     \label{tab:tn_ablation}
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{@{}l|l|l|cccc@{}}
%     \toprule
%     \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{$N$~/~$T$} \\
%     % \cmidrule(l){4-6}
%                                  &                           &                 &  6~/~10  & 8~/~30          & 16~/~60   & 32~/~100         \\ 
%     \midrule
%     \multirow{6}{*}{Mini-Kinetics} & \multirow{3}{*}{ResNet}    & Uniform   & 72.34  & 73.75  & \textbf{74.72}  & \textbf{75.15}  \\
% %                                 &                              & Random    & 72.31/89.35  & 72.52/89.62  & 74.28/90.35  & 74.84/90.75  \\
%                                  &                              & OCSampler & 73.29  & 73.52  & 74.00  & 74.17  \\
%                                  &                              & SOSampler & \textbf{73.52}  & \textbf{73.79}  & 74.46  & 74.65  \\
%     \cmidrule(l){2-7}
%                                  & \multirow{3}{*}{TimeSformer} & Uniform   & 79.77  & \textbf{80.92}  & \textbf{81.50}  & \textbf{81.61}  \\
%                                  % &                              & Random    & 79.57  & 80.01  & 80.92  & 81.68  \\
%                                  &                              & OCSampler & 80.70        & 79.13  & 78.05  & 76.33  \\
%                                  &                              & SOSampler & \textbf{80.70}        & 79.93  & 80.44  & 81.32  \\ 
%     \midrule
%     \multirow{6}{*}{COIN} & \multirow{3}{*}{ResNet} & Uniform & 78.35 & \textbf{79.86} & \textbf{81.48} & \textbf{82.88} \\
%                          % &  & Random & 77.68 & 77.52 & 80.91 & 81.67 \\
%                          &  & OCSampler & 80.15 & 78.69 & 79.79 & 80.06 \\
%                          &  & SOSampler & \textbf{80.67} & 79.13 & 80.21 & 81.02 \\
%     \cmidrule(l){2-7}
%      & \multirow{3}{*}{TimeSformer} & Uniform & 86.03 & \textbf{87.57} & \textbf{89.45} & \textbf{89.90} \\
%                                  % &  & Random & 85.00 & 85.71 & 88.58 & 89.57 \\
%                                  &  & OCSampler & 81.36 & 80.88 & 80.90 & 81.20 \\
%                                  &  & SOSampler & \textbf{87.66} & 86.52 & 87.37 & 88.08 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{0.2cm}
%     \captionof{table}{\textbf{Experiment on short video datasets for large $N$ and $T$}. The best performing model is \textbf{bold-faced}.}
%     \label{tab:short_video}
% \end{table}

==> arXiv-2409.05260v4/tables/tn_ablation_total.tex <==
\begin{table}[htbp]
    \centering
    \caption{Your Table Title}
    \label{tab:tn_ablation}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l|l|l|cccc@{}}
    \toprule
    \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{$N$~/~$T$} \\
    \cmidrule(l){4-7}
                                 &                           &                         & 6~/~10          & 8~/~30          & 16~/~60         & 32~/~100         \\ 
    \midrule
    \multirow{8}{*}{ActivityNet} & \multirow{4}{*}{ResNet}      & Uniform   & 75.41        & 77.19        & 79.45        & 80.40        \\
                                 &                              & Random    & 74.99        & 75.68        & 78.97        & 80.12        \\
                                 &                              & OCSampler & 77.20        & 78.01        & 79.10        & 80.10        \\
                                 &                              & KDSampler & 77.70        & 78.65        & 80.20        & 81.10        \\ 
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer}  & Uniform   & 87.07        & 88.51        & 89.90        & 90.30        \\
                                 &                              & Random    & 86.95        & 87.48        & 89.07        & 90.06        \\
                                 &                              & OCSampler & 83.20        & 85.06        & 85.38        & 84.53        \\
                                 &                              & KDSampler & 88.10        & 89.54        & 90.06        & 90.45        \\ 
    \midrule
    \multirow{8}{*}{Mini-Kinetics} & \multirow{4}{*}{ResNet}    & Uniform   & 72.34/89.26  & 73.75/90.14  & 74.72/90.73  & 75.15/90.80  \\
                                 &                              & Random    & 72.31/89.35  & 72.52/89.62  & 74.28/90.35  & 74.84/90.75  \\
                                 &                              & OCSampler & 73.29/89.76  & 73.52/89.99  & 74.00/90.35  & 74.17/90.55  \\
                                 &                              & KDSampler & 73.52/89.82  & 73.79/90.15  & 74.46/90.79  & 74.65/91.22  \\
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer} & Uniform   & 79.77/93.98  & 80.92/94.70  & 81.50/95.05  & 81.61/95.19  \\
                                 &                              & Random    & 79.57/94.01  & 80.01/94.18  & 80.92/94.91  & 81.68/95.01  \\
                                 &                              & OCSampler & 80.70        & 79.13/93.76  & 78.05/93.23  & 76.33/92.35  \\
                                 &                              & KDSampler & 80.70        & 79.93/93.77  & 80.44/94.70  & 81.32/94.98  \\ 
    \midrule
    \multirow{8}{*}{Mini-Sports1M} & \multirow{4}{*}{ResNet} & Uniform & 46.09 & 46.95 & 48.89 & 49.18 \\
                                 &  & Random & 45.69 & 46.09 & 48.69 & 48.92 \\
                                 &  & OCSampler & 46.7 & 48.62 & 49.62 & 50.09 \\
                                 &  & KDSampler & 48.28 & 50.00 & 51.10 & 51.46 \\
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer} & Uniform & 52.41 & 53.97 & 55.60 & 56.85 \\
                                 &  & Random & 51.67 & 52.94 & 56.55 & 57.79 \\
                                 &  & OCSampler & 47.71 & 48.93 & 49.62 & 50.03 \\
                                 &  & KDSampler & 53.75 & 55.11 & 56.85 & 57.75 \\
    \midrule
    \multirow{8}{*}{COIN} & \multirow{4}{*}{ResNet} & Uniform & 78.35 & 79.86 & 81.48 & 82.88 \\
                         &  & Random & 77.68 & 77.52 & 80.91 & 81.67 \\
                         &  & OCSampler & 80.15 & 78.69 & 79.79 & 80.06 \\
                         &  & KDSampler & 80.67 & 79.13 & 80.21 & 81.02 \\
    \cmidrule(l){2-7}
     & \multirow{4}{*}{TimeSformer} & Uniform & 86.03 & 87.57 & 89.45 & 89.90 \\
                                 &  & Random & 85.00 & 85.71 & 88.58 & 89.57 \\
                                 &  & OCSampler & 81.36 & 80.88 & 80.90 & 81.20 \\
                                 &  & KDSampler & 87.66 & 86.52 & 87.37 & 88.08 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> figures/anet_uni_oc_kd_tn_comparison.tex <==
\begin{figure}[h]
    % \vspace{}
    \centering
    \includegraphics[width=\textwidth]{files/anet_r50_uni_oc_kd_tn_comparison.png}
    \caption{\textbf{Performance by sampler across N/T.}}
    \vspace{-0.4cm}
    \label{fig:anet_comparison}
\end{figure}

==> figures/qualitative_analysis.tex <==
\begin{figure*}[th!]
    \centering
    \includegraphics[width=.74\linewidth]{files/sampled_minus.pdf}
    \vspace{0.2cm}
    \caption{\textbf{Qualitative Examples on ActivityNet-v1.3.} 
    Our approach samples only frames that are relevant to label action and contribute to downstream tasks, and discard irrelevant frames. Label action is denoted under each clip.}
    \label{fig:qualitative_analysis}
    \vspace{-0.2cm}
\end{figure*}

==> tables/3D_CNN.tex <==
\begin{table}[t]
    \centering
    % \begin{footnotesize}
    \caption{\junho{\textbf{Comparison with other methods on 3D-CNNs and Transfromers.} We perform experimental trials utilizing 3D CNNs with the aim of probing the prospect of our approach's generalizability across architectural variations. The best results are \textbf{bold-faced}.}}
    \vspace{-3mm}
    % \setlength{\tabcolsep}{0.85mm}{
    % \vspace{5pt}
    % \renewcommand\arraystretch{1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones}  & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} \\
    && mAP & GFLOPs & Top-1 &  GFLOPs \\
    \midrule
    Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    OCSampler~\cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
    KDSampler (Ours) & SlowOnly-50 & \ \ \textbf{87.5\%} & \textbf{68.2} & \textbf{82.6\%} & \textbf{2.3} \\
    %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % todo: k200 pretrained can be improved
    \midrule
    FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    OCSampler~\cite{lin2022ocsampler} & X3D-S & \ \ 86.6\% & \textbf{7.9} & \ \ -- & -- \\
    KDSampler (Ours) & X3D-S & \ \ \textbf{-\%} & \textbf{7.9} & \ \ -- & -- \\
    \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \label{tab:speed}
    % \end{footnotesize}
    \vspace{-5mm}
\end{table}


==> tables/T_ablation.tex <==
\begin{table}
    %\label{table:decision_space}
    \centering
    \resizebox{0.7\linewidth}{!}{
        \begin{tabular}{c|cccc|cccc}
        \toprule
        $T$ & \multicolumn{4}{c|}{$10$} & $6$ & $10$ & $16$ & $24$\\
        \midrule
        $N$ & $2$ & $4$ & $6$ & $8$ & \multicolumn{4}{c}{$6$}\\
        \midrule
        mAP & 71.1\% & 76.2\% & 77.7\% & \bf{77.9\%}  & 75.3\% & 77.7\% & 78.2\% & \bf{78.4\%} \\ 
        GFLOPs & \bf{9.3} & 17.6 & 25.8 & 34.1   & \bf{24.7} & 25.8 & 26.4 & 27.2 \\
        \bottomrule
        \end{tabular}
    }
    \vspace{0.2cm}
    \caption{\textbf{Ablation study on $T$ and $N$}. % $T = 6$ is same as uniform sampling.
    }
    \label{tab:t_ablation}
    \vspace{-0.3cm}
\end{table}


==> tables/ablation.tex <==
% \begin{table}[h]
% \centering
% \small
% \caption{\textbf{Ablation study on different losses on ActivityNet.} The best-performing combination is \textbf{bold-faced}.
% %of $\mathcal{L}_\text{KD}$ and $\mathcal{L}_\text{CL}$ shows the best performance.
% }
% %\vspace{-3mm}
% \begin{tabular}{ccc|c}
%     \toprule
%     $\mathcal{L}_\text{MSE}$ & $\mathcal{L}_\text{KD}$ & $\mathcal{L}_\text{CL}$  & mAP (\%)\\
%     \midrule
%     \checkmark& &  & 87.38 \\
%     % \hline
%     \checkmark&  & \checkmark &87.51 \\
%     % \hline
%     & \checkmark & & 88.21 \\
%     % \hline
%     & \checkmark & \checkmark & \textbf{88.65} \\
%     \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:loss_ablation}
% \end{table}

\begin{table}
    \centering
    \footnotesize
    % \vspace{-3mm}
    \begin{tabular}{cccc|c|c}
        \toprule
        % $\mathcal{L}_{MSE}$ & $\mathcal{L}_{KD}$ & $\mathcal{L}_{CL}$  & mAP (\%)\\
        \multicolumn{4}{c|}{$\bm{\mathcal{L}_\text{KD}}$}  & \multirow{2}{*}{\bm{$\mathcal{L}_\text{CE}$}}  & \multirow{2}{*}{mAP (\%)}\\
        % MSE & Ranking Loss & $\mathcal{L}_{CL}$  & mAP (\%)\\
        % \midrule
        MSE         & Ranking   & Label     & Max           &           & \\
        \midrule
        \checkmark &             &  \checkmark   &           &              &   87.38 \\
        \checkmark &             &  \checkmark   &           & \checkmark   & 87.51 \\
                   & \checkmark  & \checkmark    &           &              & 88.21 \\
                   & \checkmark  &  \checkmark   &           &  \checkmark  & 88.40 \\
                  &\checkmark &                  &  \checkmark    &  \checkmark &\textbf{88.65} \\
        % \hline
        \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \caption{\textbf{Ablation study on different losses on ActivityNet.}}
    \label{tab:loss_ablation}
\end{table}

==> tables/anet_x3d.tex <==
\begin{table}[t]
    \caption{\textbf{X3D-S Comparison on ActivityNet}.} % $T = 6$ is same as uniform sampling.
    \vspace{-3mm}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{l|cc}
        \toprule
        Method & mAP & GFLOPs\\
        \midrule
        Baseline & 65.1\% & - \\
        OCSampler~\cite{lin2022ocsampler} & 66.3\% & 7.9 \\
        \textbf{KDSampler} & \textbf{68.5\%} & 7.9 \\ 
        \textbf{KDSampler} & 67.1\% & \textbf{7.5} \\ 
        \bottomrule
    \end{tabular}
    }
    \label{table:anet_x3d}
    \vspace{-5mm}
\end{table}


==> tables/large_t_n.tex <==

\begin{table}
    \caption{\textbf{Comparison with large $T$ and $N$}.}
    % \vspace{-3mm}
    \footnotesize
    \centering
        \begin{tabular}{l|cccc}
        \toprule
        \multicolumn{1}{c|}{$T$} & 30 & 60 & 100 & 100 \\
        \multicolumn{1}{c|}{$N$} & 16 & 16 & 16 & 32 \\
        \midrule
        Uniform sampler & 79.2\% & 79.2\% & 79.2\% & 80.2\% \\
        OCSampler~\cite{lin2022ocsampler} & 78.6\% & 78.2\% & 77.9\% & 79.2\% \\
        KDSampler (Ours) & \textbf{80.0\%} & \textbf{80.2\%} & \textbf{80.5\%} & \textbf{81.0\%} \\
        \bottomrule
        \end{tabular}
    \label{tab:ablation_t_n_large}
    % \vspace{-2mm}
\end{table}


==> tables/oracle_conf_indice.tex <==
\begin{table}
    \centering
    \caption{\textbf{Sampling Fidelity}. 
    Note that we report the expected value of the sampling fidelity for random sampling.
    % We report the sampling fidelity, which indicates the similarity of the sampled set to the oracle set, across various values of $N$. Note that we report the expected value of the sampling fidelity for random sampling. All the policies employ the same classifier and frame candidates, with $T$ fixed at 10.
    }
    \label{tab:fidelity}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|c|cccccc}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampler} & \multicolumn{6}{c}{Sampling Fidelity} \\ 
                             &                          & $N=$~1& $N=$~2& $N=$~3& $N=$~4& $N=$~5& $N=$~6    \\ \midrule
    \multirow{3}{*}{ActivityNet} & Random                 & 0.100  & 0.200  & 0.300  & 0.400  & 0.500 & 0.600  \\ 
                             & FrameExit                & 0.102 & 0.193 & 0.293 & 0.393 & 0.496 & 0.593\\ %\cline{2-8} 
                             & $\pi_s$                      & 1.000    & 0.74 & 0.73 & 0.75 & 0.78 & 0.81 \\ \midrule
    \multirow{3}{*}{Mini-Kinetics} & Random                & 0.100  & 0.200  & 0.300  & 0.400  & 0.500  & 0.600 \\
                             & FrameExit                & 0.098& 0.225& 0.320& 0.425& 0.515& 0.625\\ %\cline{2-8} 
                             & $\pi_s$                     & 1.00    & 0.61 & 0.65 & 0.70  & 0.71  & 0.80  \\ 
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.3cm}
\end{table}

% \begin{table}[h]
% \centering
% \caption{Number of Sampled Frames Data}
% \label{tab:sampled_frames}
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%     \hline
%     \multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampler} & \multicolumn{6}{c|}{Number of sampled frames} \\ \cline{3-8} 
%                              &                          & 1    & 2    & 3    & 4    & 5    & 6    \\ \hline
%     \multirow{3}{*}{ActivityNet} & Random                 & 0.1  & 0.2  & 0.3  & 0.4  & 0.5  & 0.6  \\ \cline{2-8} 
%                              & FrameExit                & 0.099& 0.225& 0.32 & 0.425& 0.515& 0.625\\ \cmidrule{3-8} 
%                              & S\_c                      & 1    & 0.74 & 0.73 & 0.75 & 0.78 & 0.81 \\ \hline
%     \multirow{3}{*}{Mini-Kinetics} & Random                & 0.1  & 0.2  & 0.3  & 0.4  & 0.5  & 0.6  \\ \cline{2-8} 
%                              & FrameExit                & 0.101& 0.193& 0.293& 0.393& 0.496& 0.593\\ \cmidrule{3-8} 
%                              & S\_c                      & 1    & 0.61 & 0.65 & 0.7  & 0.7  & 0.8  \\ \hline
%     \end{tabular}
% \end{table}

==> tables/oracle_conf_perform.tex <==
\begin{table}
    \begin{center}
    \caption{\textbf{Performance of $\pi_o$ and $\pi_s$ on ActivityNet-v1.3 and Mini-Kinetics}. \junho{Relative improvement from $\pi_u$ is provided on the right side.}
    % We report the performance of the classifier, depending on the different sampling policies of the uniform policy $\pi_u$, oracle policy $\pi_o$, semi-optimal policy $\pi_s$, and input all candidate frames. (Relative improvement from $\pi_u$ is provided as well.) Given $T=10$ candidate frames, each policy selects $N=6$ frames using their sampling policy. Note that classifiers are fixed and only the sampling policy is varied. The results indicate that $\pi_s$ can effectively approximate $\pi_o$ for all benchmarks.
    }
    \vspace{-0.2cm}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|c|cr|cr}
        \toprule
        $f_c$ & Policy & \multicolumn{2}{c|}{ActivityNet (mAP)} & \multicolumn{2}{c}{Mini-Kinetics (Top-1)} \\
        %\midrule 
        %\multicolumn{3}{c}{\textit{ResNet50}} \\
        \midrule
        \multirow{4}{*}{TimeSformer} & $\pi_u$ & 87.09\% & -- & 79.62\% & --\\
        & $\pi_o$ &  91.59\% & +4.50 & 89.36\% & +9.66\\
        & $\pi_s$ &  89.35\% & +2.26 & 84.77\% & +5.15\\
        & All & 89.00\% & +1.91 & 81.23\% & +1.61\\
        \midrule
        \multirow{4}{*}{ResNet50} & $\pi_u$ & 75.33\% & -- & 72.54\% & -- \\
        & $\pi_o$ &  90.54\% & +15.21 & 83.84\% & +11.30 \\
        & $\pi_s$ &  87.44\% & +12.11 & 80.27\% & +7.73 \\
        & All & 77.89\% & +2.56 & 73.64\% & +1.10 \\
        %\midrule 
        %\multicolumn{3}{c}{\textit{TimeSformer}} \\
        \bottomrule
        \end{tabular}
    }
    \vspace{-0.6cm}
    \label{tab:oracle_conf_sampler_result}
    \end{center} 
\end{table}

==> tables/resnet_anet_minik_sota.tex <==
% \begin{table}[t]
%     \centering
%     % \begin{footnotesize}
%     \caption{\textbf{Comparison on ActivityNet-v1.3 and Mini-Kinetics.} The best performing model is \textbf{bold-faced}.}
%     \label{table:sota_anet_k200}
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{l|c|cccccccccc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} &  \multicolumn{2}{c}{Mini-Sports1M} &  \multicolumn{2}{c}{COIN} \\
%     & & mAP & GFLOPs & Top-1 &  GFLOPs & mAP & GFLOPs & mAP & GFLOPs\\
%     \midrule
%     %AdaFrame \cite{wu2019adaframe} & ResNet & \ \ 71.5\% & 79.0 & \ \ -- & -- \\
%     %ListenToLook \cite{gao2020listen} & ResNet & \ \ 72.3\%  & 81.4 & -- & -- \\
%     LiteEval \cite{wu2019liteeval}& \multirow{8}{*}{ResNet} & \ \ 72.7\% & 95.1 & \ \ 61.0\% & 99.0 &  44.7\%  & 66.2  & -- & --\\ 
%     SCSampler \cite{korbar2019scsampler}& & \ \ 72.9\%  & 42.0 & \ \ 70.8\% & 41.9 & 44.3\% & 42.0 & 73.89\% & 42.0 \\
%     AR-Net \cite{meng2020arnet}& & \ \ 73.8\% & 33.5 & \ \ 71.7\% & 32.0 & 45.0\% & 37.6 & -- & -- \\
%     AdaFuse \cite{meng2021adafuse} & & -- & -- & -- & -- &  44.1\% & 60.3 & -- & -- \\
%     videoIQ \cite{sun2021videoiq}& & \ \ 74.8\% & 28.1 & \ \ 72.3\% & 20.4 & -- & -- & -- & -- \\
%     AdaFocus \cite{wang2022adafocus}& & \ \ 75.0\% & 26.6 & \ \ 72.9\% & 38.6 & -- & -- & -- & -- \\
%     FrameExit \cite{ghodrati2021frameexit}& & \ \ 76.1\% & 26.1 & \ \ 72.8\% & \bf{19.7} & -- & -- & -- & -- \\
%     % \rowcolor{lavendergray}\textit{Samples from 10 to N} & & & &  \\
%     OCSampler \cite{lin2022ocsampler}& & \ \ 77.2\% & \textbf{25.8} & \ \ 73.0\% & {21.6} & 46.7\% & 25.7 & 74.28\% & 25.8 \\
%                                       % & \ \ 76.9\% (5) & 21.7 & \ \ 72.25\% (4) & 17.5 \\
%     \textbf{KDSampler} && \ \ {\textbf{77.7\%}}& \textbf{25.8} & \ \  {\textbf{73.5\%}}& {21.6} &{\textbf{47.5\%}} & 25.7 & {\textbf{74.89\%}} & 25.8\\
%                      % & \ \ \junho{77.3\%} (5) & 21.7 & \ \  \junho{72.49\%} (4) & 17.5 \\
%     \midrule
%     % Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
%     % OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
%     Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 & \ \ -- & --  & \ \ -- & --\\
%     OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & 68.2 & 82.6\% & 27.3 & \ \ -- & --  & \ \ -- & --\\
%     \textbf{KDSampler} &  & \ \ \textbf{88.0\%} & \textbf{64.0} & \textbf{83.0\%} & 27.3 & \ \ -- & --  & \ \ -- & --\\
%     %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
%     % todo: k200 pretrained can be improved
%     \midrule
%     FrameExit \cite{ghodrati2021frameexit} & \multirow{3}{*}{X3D-S} & \ \ 86.0\% & 9.8 & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     OCSampler~\cite{lin2022ocsampler} &  & \ \ 86.6\% & 7.9 & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     \textbf{KDSampler} &  & \ \ {\textbf{87.2\%}} & {\textbf{7.6}} & \ \ -- & -- & \ \ -- & --  & \ \ -- & -- \\
%     \midrule
%     % Uniform  & \multirow{3}{*}{TimeSformer} & \ \ 87.1\% & \bf{75.7} & \ \ 79.6\% & \bf{75.7} \\
%     OCSampler~\cite{lin2022ocsampler} & \multirow{2}{*}{TimeSformer} & \ \ 83.2\% & {76.8} & \ \ 80.7\% & {76.8} & 45.69\% & 76.77 & 79.27\% & 76.77\\
%     \textbf{KDSampler} &  & \ \ \textbf{88.1\%} & \textbf{64.16} & \ \ 80.7\% & {76.8} & \textbf{49.05\%} & \textbf{64.16} & \textbf{80.81\%} & \textbf{64.16} \\
%     \bottomrule
%     % \rowcolor{gray}\textit{Kinetics} & & & & &\\
%     % Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
%     % ListenToLook \cite{gao2020listentolook} & R(2+1)D-152 & \ \ 89.9\% & 2640 & -- & -- \\
%     % MARL \cite{wu2019marl} & SEResNeXt-152 & \ \ 90.0\% & 7540 & -- & -- \\
%     % OCSampler \cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & \textbf{82.6\%} & \textbf{27.3} \\
%     % %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
%     % OCSampler \cite{lin2022ocsampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 593 & - & - \\
    
%     % % todo: k200 pretrained can be improved
%     % \hline
%     % \rowcolor{gray}\textit{Kinetics} & & & & &\\
%     % FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
%     % OCSampler \cite{lin2022ocsampler} & X3D-S & \ \ \textbf{86.6\%} & \textbf{7.9} & \ \ -- & -- \\
%     \end{tabular}
%     }
%     % \vspace{-0.6cm}
% \end{table}

\begin{table}[t]
    \centering
    % \begin{footnotesize}
    \caption{\textbf{Comparison on ActivityNet-v1.3 and Mini-Kinetics.} The best performing model is \textbf{bold-faced}.}
    \label{table:sota_anet_k200}
    % \vspace{-3mm}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} \\
    & & mAP & GFLOPs & Top-1 &  GFLOPs \\
    \midrule
    %AdaFrame \cite{wu2019adaframe} & ResNet & \ \ 71.5\% & 79.0 & \ \ -- & -- \\
    %ListenToLook \cite{gao2020listen} & ResNet & \ \ 72.3\%  & 81.4 & -- & -- \\
    LiteEval \cite{wu2019liteeval}& \multirow{8}{*}{ResNet} & \ \ 72.7\% & 95.1 & \ \ 61.0\% & 99.0  \\ 
    SCSampler \cite{korbar2019scsampler}& & \ \ 72.9\%  & 42.0 & \ \ 70.8\% & 41.9 \\
    AR-Net \cite{meng2020arnet}& & \ \ 73.8\% & 33.5 & \ \ 71.7\% & 32.0 \\
    videoIQ \cite{sun2021videoiq}& & \ \ 74.8\% & 28.1 & \ \ 72.3\% & 20.4 \\
    AdaFocus \cite{wang2022adafocus}& & \ \ 75.0\% & 26.6 & \ \ 72.9\% & 38.6 \\
    FrameExit \cite{ghodrati2021frameexit}& & \ \ 76.1\% & 26.1 & \ \ 72.8\% & \bf{19.7} \\
    % \rowcolor{lavendergray}\textit{Samples from 10 to N} & & & &  \\
    OCSampler \cite{lin2022ocsampler}& & \ \ 77.2\% & \textbf{25.8} & \ \ 73.0\% & {21.6} \\
                                      % & \ \ 76.9\% (5) & 21.7 & \ \ 72.25\% (4) & 17.5 \\
    \textbf{KDSampler} && \ \ {\textbf{77.7\%}}& \textbf{25.8} & \ \  {\textbf{73.5\%}}& {21.6} \\
                     % & \ \ \junho{77.3\%} (5) & 21.7 & \ \  \junho{72.49\%} (4) & 17.5 \\
    \midrule
    % Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    % OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & \textbf{68.2} & 82.6\% & \textbf{27.3} \\
    Ada2D \cite{li2021ada2d} & \multirow{3}{*}{SlowOnly-50} & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    OCSampler~\cite{lin2022ocsampler} &  & \ \ 87.3\% & 68.2 & 82.6\% & 27.3 \\
    \textbf{KDSampler} &  & \ \ \textbf{88.0\%} & \textbf{64.0} & \textbf{83.0\%} & 27.3 \\
    %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % todo: k200 pretrained can be improved
    \midrule
    FrameExit \cite{ghodrati2021frameexit} & \multirow{3}{*}{X3D-S} & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    OCSampler~\cite{lin2022ocsampler} &  & \ \ 86.6\% & 7.9 & \ \ -- & -- \\
    \textbf{KDSampler} &  & \ \ {\textbf{87.2\%}} & {\textbf{7.6}} & \ \ -- & -- \\
    \midrule
    % Uniform  & \multirow{3}{*}{TimeSformer} & \ \ 87.1\% & \bf{75.7} & \ \ 79.6\% & \bf{75.7} \\
    OCSampler~\cite{lin2022ocsampler} & \multirow{2}{*}{TimeSformer} & \ \ 83.2\% & {76.8} & \ \ 80.7\% & {76.8} \\
    \textbf{KDSampler} &  & \ \ \textbf{88.1\%} & \textbf{64.16} & \ \ 80.7\% & {76.8} \\
    \bottomrule
    % \rowcolor{gray}\textit{Kinetics} & & & & &\\
    % Ada2D \cite{li2021ada2d} & SlowOnly-50 & \ \ 84.0\% & 701 & 79.2\% & 738 \\
    % ListenToLook \cite{gao2020listentolook} & R(2+1)D-152 & \ \ 89.9\% & 2640 & -- & -- \\
    % MARL \cite{wu2019marl} & SEResNeXt-152 & \ \ 90.0\% & 7540 & -- & -- \\
    % OCSampler \cite{lin2022ocsampler} & SlowOnly-50 & \ \ 87.3\% & \textbf{68.2} & \textbf{82.6\%} & \textbf{27.3} \\
    % %\textbf{OCSampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 308 & \textbf{82.4\%} & 54.7 \\
    % OCSampler \cite{lin2022ocsampler} & SlowOnly-101 & \ \ \textbf{90.1\%} & 593 & - & - \\
    
    % % todo: k200 pretrained can be improved
    % \hline
    % \rowcolor{gray}\textit{Kinetics} & & & & &\\
    % FrameExit \cite{ghodrati2021frameexit} & X3D-S & \ \ 86.0\% & 9.8 & \ \ -- & -- \\
    % OCSampler \cite{lin2022ocsampler} & X3D-S & \ \ \textbf{86.6\%} & \textbf{7.9} & \ \ -- & -- \\
    \end{tabular}
    }
    % \vspace{-0.6cm}
\end{table}

==> tables/resnet_minis_fcvid_coin_sota.tex <==
\begin{table}
    \begin{center}
    \caption{\textbf{Comparison with competing models on Mini-Sports1M and COIN}. The best performing model is \textbf{bold-faced}.}
    % \vspace{-2mm}
    \resizebox{0.5\linewidth}{!}{
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|@{\hspace{0.4cm}}cccc}
        \toprule
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Backbones} & \multicolumn{2}{c}{Mini-Sports1M} &  \multicolumn{2}{c}{COIN} \\
        & & mAP & GFLOPs & Top-1 &  GFLOPs \\
        % \midrule
        % ResNet50 &&&& \\
        \midrule        
        LiteEval~\cite{wu2019liteeval}& \multirow{6}{*}{ResNet50} & 44.7\% & 66.2 & - & - \\
        SCSampler~\cite{korbar2019scsampler} && 44.3\% & 42.0 & 73.89\% & 42.0 \\
        AR-Net~\cite{meng2020arnet} && 45.0\% & 37.6 & - & - \\
        AdaFuse~\cite{meng2021adafuse} &&  44.1\% & 60.3 & - & - \\ %
        OCSampler~\cite{lin2022ocsampler} && 46.7\% & 25.7 & 74.28\% & 25.8 \\
        % \midrule
        \textbf{KDSampler} (ours) &&{\textbf{47.5\%}} & 25.7 & {\textbf{74.89\%}} & 25.8 \\
        % \midrule
        % TimeSformer &&&& \\
        \midrule
        % Uniform  & \multirow{3}{*}{TimeSfromer} & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        OCSampler \cite{lin2022ocsampler} & \multirow{2}{*}{TimeSfromer}& 45.69\% & 76.77 & 79.27\% & 76.77  \\
        \textbf{KDSampler} (ours) && \textbf{49.05\%} & \textbf{64.16} & \textbf{80.81\%} & \textbf{64.16} \\
        \bottomrule
        \end{tabular}
    } 
    \vspace{-2mm}
    \label{table:sota_sport_coin}
    \end{center} 
    \vspace{-2mm}
\end{table}

% \begin{table}
%     \begin{center}
%     \caption{\small \textbf{Improvement comparison from baseline on Mini-Sports1M and FCVID}. OCSampler achieves the best mAP while offering significant savings in GFLOPs.}
%     \vspace{-2mm}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccccc}
%         \hline
%         \multirow{2}{*}{Methods} &  \multicolumn{2}{c}{Mini-Sports1M} & \multicolumn{2}{c}{FCVID} & \multicolumn{2}{c}{COIN}  \\
%         &  mAP & GFLOPs  &  mAP & GFLOPs  &  Top-1 & GFLOPs \\
%         \hline 
%         \hline 
%         Baseline (ResNet50) & 39.98\% & 24.7 & --\% & 24.7 & 73.91 & 24.7 \\
%         OCSampler \cite{lin2022ocsampler} & --\% & 25.8 & --\% & 25.8 & 74.28 & 25.8 \\
%         KDSampler  & 40.87\% & 25.8 & --\% & 25.8 & 74.89 & 25.8 \\
%         % LiteEval~\cite{wu2019liteeval} & 44.7\% & 66.2 & 80.0\% & 94.3 \\
%         % SCSampler~\cite{korbar2019scsampler} & 44.3\% & 42.0 & 81.0\% & 42.0 \\
%         % AR-Net~\cite{meng2020ar} & 45.0\% & 37.6 & 81.3\% & 35.1 \\
%         % AdaFuse~\cite{meng2020adafuse} &  44.1\% & 60.3 & 81.6\% & 45.0 \\ %
%         % \hline
%         \hline
%         \end{tabular}
%     } 
%     \vspace{-2mm}
%     \label{table:sota_actv_fcvid}
%     \end{center} 
%     %\vspace{-5mm}
% \end{table}

==> tables/timesformer.tex <==
\begin{table*}
    \vspace{-0.2cm}
    \begin{center}
    \caption{
    \textbf{Comparison with TimeSformer Classifiers.} We report performance of our approach compared to uniform sampling and OCSampler \cite{lin2022ocsampler}, which is the SOTA frame sampler in CNN architecture on ActivityNet-v1.3, Mini-Kinetics, Mini-Sports1M, and COIN. Although OCSampler works well with CNNs, it fails to outperform even uniform sampling with Transformer classifiers except on Mini-Kinetics dataset. However, our approach shows great performance on all datasets with the Transformer architecture. 
    % However, our apporoach still do not approach to teacher sampler $S_c$
    }
    \vspace{-0.2cm}
    \begin{footnotesize}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccccc}
        \toprule
        \multirow{2}{*}{Methods (T/N)} & \multicolumn{2}{c}{ActivityNet} &  \multicolumn{2}{c}{Mini-Kinetics} &  \multicolumn{2}{c}{Mini-Sports1M} & \multicolumn{2}{c}{COIN} \\
        & mAP & GFLOPs & Top-1 & GFLOPs & mAP & GFLOPs & Top-1 & GFLOPs\\
        \midrule
        Uniform (6/-) & 87.09\% & 75.73G & 79.62\% & 75.73G & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        % Uniform (10/-) & 87.09\% & 75.73G & 79.62\% & 75.73G & 48.90\% & 75.73G &  79.88\% & 75.73G \\
        OCSampler (6/10) \cite{lin2022ocsampler} & 83.20\% & 76.77G & \textbf{80.66\%} & 76.77G & 45.69\% & 76.77G &  79.27\% & 76.77G \\
        KDSampler (5/10) & 88.13\% & 64.16G & 79.75\% & 64.16G & 49.05\% & 64.16G & 80.81\% & 64.16G \\
        ~~~~~~~~~~~~~~~~~~~ (6/10) & \textbf{88.65\%} & 76.77G & 80.52\% & 76.77G & \textbf{50.04\%} & 76.77G &  \textbf{81.62\%} & 76.77G\\
        % \midrule
        
        \bottomrule
        \end{tabular}
    %} 
    \vspace{-0.4cm}
    \label{table:timesformer_sota}
    \end{footnotesize}
    \end{center} 
\end{table*}

==> tables/tn_ablation_anet_minis.tex <==
\begin{table}[htbp]
    \centering
    \label{tab:tn_ablation}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{@{}l|l|l|ccc@{}}
    \toprule
    \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{$N$~/~$T$} \\
    % \cmidrule(l){4-6}
                                 &                           &         & 8~/~30          & 16~/~60         & 32~/~100         \\ 
    \midrule
    \multirow{6}{*}{ActivityNet} & \multirow{4}{*}{ResNet}      & Uniform           & 77.19        & 79.45        & 80.40        \\
                                 % &                              & Random            & 75.68        & 78.97        & 80.12        \\
                                 &                              & OCSampler         & 78.01        & 79.10        & 80.10        \\
                                 &                              & KDSampler         & \textbf{78.65}        & \textbf{80.20}        & \textbf{81.10}        \\ 
    \cmidrule(l){2-6}
                                 & \multirow{4}{*}{TimeSformer}  & Uniform           & 88.51        & 89.90        & 90.30        \\
                                 % &                              & Random            & 87.48        & 89.07        & 90.06        \\
                                 &                              & OCSampler         & 85.06        & 85.38        & 84.53        \\
                                 &                              & KDSampler         & \textbf{89.54}        & \textbf{90.06}        & \textbf{90.45}        \\ 
    \midrule
    \multirow{6}{*}{Mini-Sports1M} & \multirow{4}{*}{ResNet} & Uniform  & 46.95 & 48.89 & 49.18 \\
                                 % &  & Random  & 46.09 & 48.69 & 48.92 \\
                                 &  & OCSampler  & 48.62 & 49.62 & 50.09 \\
                                 &  & KDSampler  & \textbf{50.00} & \textbf{51.10} & \textbf{51.46} \\
    \cmidrule(l){2-6}
                                 & \multirow{4}{*}{TimeSformer} & Uniform  & 53.97 & 55.60 & 56.85 \\
                                 % &  & Random  & 52.94 & 56.55 & 57.79 \\
                                 &  & OCSampler & 48.93 & 49.62 & 50.03 \\
                                 &  & KDSampler & \textbf{55.11} & \textbf{56.85} & \textbf{57.75} \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Experiment on long video datasets for large $T$ and $N$}. The best performing model is \textbf{bold-faced}.}
\end{table}


==> tables/tn_ablation_total.tex <==
\begin{table}[htbp]
    \centering
    \caption{Your Table Title}
    \label{tab:tn_ablation}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l|l|l|cccc@{}}
    \toprule
    \multirow{2}{*}{Dataset}     & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{$N$~/~$T$} \\
    \cmidrule(l){4-7}
                                 &                           &                         & 6~/~10          & 8~/~30          & 16~/~60         & 32~/~100         \\ 
    \midrule
    \multirow{8}{*}{ActivityNet} & \multirow{4}{*}{ResNet}      & Uniform   & 75.41        & 77.19        & 79.45        & 80.40        \\
                                 &                              & Random    & 74.99        & 75.68        & 78.97        & 80.12        \\
                                 &                              & OCSampler & 77.20        & 78.01        & 79.10        & 80.10        \\
                                 &                              & KDSampler & 77.70        & 78.65        & 80.20        & 81.10        \\ 
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer}  & Uniform   & 87.07        & 88.51        & 89.90        & 90.30        \\
                                 &                              & Random    & 86.95        & 87.48        & 89.07        & 90.06        \\
                                 &                              & OCSampler & 83.20        & 85.06        & 85.38        & 84.53        \\
                                 &                              & KDSampler & 88.10        & 89.54        & 90.06        & 90.45        \\ 
    \midrule
    \multirow{8}{*}{Mini-Kinetics} & \multirow{4}{*}{ResNet}    & Uniform   & 72.34/89.26  & 73.75/90.14  & 74.72/90.73  & 75.15/90.80  \\
                                 &                              & Random    & 72.31/89.35  & 72.52/89.62  & 74.28/90.35  & 74.84/90.75  \\
                                 &                              & OCSampler & 73.29/89.76  & 73.52/89.99  & 74.00/90.35  & 74.17/90.55  \\
                                 &                              & KDSampler & 73.52/89.82  & 73.79/90.15  & 74.46/90.79  & 74.65/91.22  \\
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer} & Uniform   & 79.77/93.98  & 80.92/94.70  & 81.50/95.05  & 81.61/95.19  \\
                                 &                              & Random    & 79.57/94.01  & 80.01/94.18  & 80.92/94.91  & 81.68/95.01  \\
                                 &                              & OCSampler & 80.70        & 79.13/93.76  & 78.05/93.23  & 76.33/92.35  \\
                                 &                              & KDSampler & 80.70        & 79.93/93.77  & 80.44/94.70  & 81.32/94.98  \\ 
    \midrule
    \multirow{8}{*}{Mini-Sports1M} & \multirow{4}{*}{ResNet} & Uniform & 46.09 & 46.95 & 48.89 & 49.18 \\
                                 &  & Random & 45.69 & 46.09 & 48.69 & 48.92 \\
                                 &  & OCSampler & 46.7 & 48.62 & 49.62 & 50.09 \\
                                 &  & KDSampler & 48.28 & 50.00 & 51.10 & 51.46 \\
    \cmidrule(l){2-7}
                                 & \multirow{4}{*}{TimeSformer} & Uniform & 52.41 & 53.97 & 55.60 & 56.85 \\
                                 &  & Random & 51.67 & 52.94 & 56.55 & 57.79 \\
                                 &  & OCSampler & 47.71 & 48.93 & 49.62 & 50.03 \\
                                 &  & KDSampler & 53.75 & 55.11 & 56.85 & 57.75 \\
    \midrule
    \multirow{8}{*}{COIN} & \multirow{4}{*}{ResNet} & Uniform & 78.35 & 79.86 & 81.48 & 82.88 \\
                         &  & Random & 77.68 & 77.52 & 80.91 & 81.67 \\
                         &  & OCSampler & 80.15 & 78.69 & 79.79 & 80.06 \\
                         &  & KDSampler & 80.67 & 79.13 & 80.21 & 81.02 \\
    \cmidrule(l){2-7}
     & \multirow{4}{*}{TimeSformer} & Uniform & 86.03 & 87.57 & 89.45 & 89.90 \\
                                 &  & Random & 85.00 & 85.71 & 88.58 & 89.57 \\
                                 &  & OCSampler & 81.36 & 80.88 & 80.90 & 81.20 \\
                                 &  & KDSampler & 87.66 & 86.52 & 87.37 & 88.08 \\
    \bottomrule
    \end{tabular}
    }
\end{table}
